Algorithmic Randomness, Effective Disintegrations, and Rates of Convergence to the Truth

L\'evy's Upward Theorem says that the conditional expectation of an integrable random variable converges with probability one to its true value with increasing information. In this paper, we use methods from effective probability theory to characterise the probability one set along which convergence to the truth occurs, and the rate at which the convergence occurs. We work within the setting of computable probability measures defined on computable Polish spaces and introduce a new general theory of effective disintegrations. We use this machinery to prove our main results, which (1) identify the points along which certain classes of effective random variables converge to the truth in terms of certain classes of algorithmically random points, and which further (2) identify when computable rates of convergence exist. Our convergence results significantly generalize earlier results within a unifying novel abstract framework, and there are no precursors of our results on computable rates of convergence. Finally, we make a case for the importance of our work for the foundations of Bayesian probability theory.

==> 12-maximal-function.tex <==
\section{Classical features of the maximal function}\label{sec:maximal:classical}

Suppose that $\nu$ is a point of $\mathcal{P}(X)$ and $\mathscr{F}_n$ is any increasing filtration of Borel subsets of $X$. In this section, we recall some classical features of the maximal function $f^{\ast}=\sup_n \mathbb{E}_{\nu}[f\mid \mathscr{F}_n]$ of an integrable function $f$.

First, we recall the following, which tells gives us information about the codomain of the maximal function:
\begin{lem}\label{lem:doob}
\item[]
\begin{enumerate}[leftmargin=*]
\item If $p>1$ then  $\|g^{\ast}\|_p\leq \frac{p}{p-1} \cdot \|g\|_p$ for $g$ in $L_p^+(\nu)$, and the maximal function maps $L_p(\nu)$ to $L_p(\nu)$.
\item If $p=1$, then the maximal function maps $L_p(\nu)$ to $L_0(\nu)$.
\end{enumerate}
\end{lem}
\begin{proof}
For $p>1$, the sequence $\mathbb{E}_{\nu}[g\mid \mathscr{F}_n]$ is a non-negative martingale, and so by Doob's Maximal Inequality\footnote{\cite[Theorem 9.4 pp. 505-506]{Gut2013-ou}.}  followed by conditional Jensen we have: $\|\sup_{n\leq m} \mathbb{E}_{\nu}[g\mid \mathscr{F}_n]\|_p\leq \frac{p}{p-1}\cdot  \|\mathbb{E}_{\nu}[g\mid \mathscr{F}_m]\|_p\leq \frac{p}{p-1} \cdot \|g\|_p$. Since these are non-negative functions, by the Monotone Convergence Theorem we have $\|g^{\ast}\|_p\leq \frac{p}{p-1} \|g\|_p$. For $p=1$, let $\mathscr{F}_{\infty}$ be the $\sigma$-algebra generated by all the $\mathscr{F}_n$. 
By the classical L\'evy Upward Theorem we have that $\mathbb{E}_{\nu}[g\mid \mathscr{F}_n]\rightarrow \mathbb{E}_{\nu}[g\mid \mathscr{F}_{\infty}]$ $\nu$-a.s. which shows that $g^{\ast}$ is finite $\nu$-a.s., and hence that $g^{\ast}$ is in $L_0(\nu)$.
\end{proof}

Some of the salient properties of the maximal function are captured by the notion of a monotone sublinear map.\footnote{For these definitions, see \cite[181, 283]{Aliprantis2013-ep}.} Let $K$ be a subfield of the reals. Suppose  $X,Y$ are two ordered $K$-vector spaces. A map $\varphi:X\rightarrow Y$ is \emph{sublinear} if it satisfies both
\begin{itemize}[leftmargin=*]
\item $\varphi(\lambda \cdot x)=\lambda \cdot \varphi(x)$ and $\varphi(x+x^{\prime})\leq \varphi(x)+\varphi(x^{\prime})$ for $\lambda\geq 0$ in $K$ and $x,x^{\prime}$ in $X$.
\end{itemize}
And $\varphi:X\rightarrow Y$ is \emph{monotone} if it satisfies 
\begin{itemize}[leftmargin=*]
\item $x\leq x^{\prime}$ implies $\varphi(x)\leq \varphi(x^{\prime})$ for all $x,x^{\prime}$ in $X$.
\end{itemize}
Further, a subset $P\subseteq X^+$ is a \emph{positive cone} if it satisfies
\begin{itemize}[leftmargin=*]
\item $\lambda \cdot x+\lambda^{\prime} \cdot x^{\prime}$ in $P$ for all $x,x^{\prime}$ in $P$ and $\lambda, \lambda^{\prime}\geq 0$ in $K$.
\end{itemize}
The notion of $\varphi:P\rightarrow Y$ being (monotone) sublinear is defined by relativisation, and any (monotone) sublinear map $\varphi:X\rightarrow Y$ induces a (montone) sublinear map $\varphi\upharpoonright P :P\rightarrow Y$ by restriction.  If $X$ is a Riesz space (i.e. a lattice induces the partial order), then a sublinear map $\varphi:X\rightarrow Y$ satisfies \emph{the reverse triangle inequality}: 
\begin{itemize}[leftmargin=*]
\item $\left|\varphi(x)-\varphi(y)\right|\leq \varphi(\left|x-y\right|)$. 
\end{itemize}
Simple examples of montone sublinear maps are the conditional expectation operators from $L_p(\nu)$ to itself, and the norm $\|\cdot\|:X^+\rightarrow \mathbb{R}$ when $X$ is a normed Riesz space (i.e. a Riesz space which is normed and satisfies: if $\left|x\right|\leq \left|x^{\prime}\right|$ then $\|x\|\leq \|x^{\prime}\|$). The other examples, like the maximal function itself, come from taking a supremum of countably many monotone sublinear maps:
\begin{itemize}[leftmargin=*]
\item If $\varphi_n:X\rightarrow Y$ is monotone sublinear and $\sup_n \varphi_n(x)$ exists in $Y$ for any $x$ from $X$, then $\sup_n \varphi_n:X\rightarrow Y$ is monotone sublinear. And similarly when restricted to a positive cone in~$X$.
\end{itemize}
\noindent (In $\sup_n \varphi_n(x)$, the supremum is given in the sense of partial order on $Y$).

The following collects together all the classical facts about the maximal function which we need:
\begin{prop}\label{prop:abstract:1}\mbox{\;}
\begin{enumerate}[leftmargin=*]
    \item \label{prop:abstract:1a} For $p>1$, the maximal function ${\cdot}^{\ast}: L_p(\nu) \rightarrow L_p(\nu)$ is monotone sublinear and uniformly continuous with modulus $m(\epsilon)=\frac{p-1}{p}\cdot \epsilon$ of uniform continuity.
    \item \label{prop:abstract:1b} For $p=1$, the maximal function ${\cdot}^{\ast}: L_p(\nu) \rightarrow L_0(\nu)$ is monotone sublinear and uniformly continuous with a modulus $m(\epsilon)=\epsilon^2$ of uniform continuity.
\end{enumerate}
\end{prop}
\begin{proof}
The montone sublinearity follows from the observation about supremums.

Let $p>1$ and $f$ in $L_p(\nu)$. By Lemma~\ref{lem:doob} one has for $f,g$ in $L_p(\nu)$ with $\|f-g\|_p<\frac{p-1}{p}\cdot \epsilon$ that $\|f^{\ast}-g^{\ast}\|_p\leq \|\left|f-g\right|^{\ast}\|_p\leq \frac{p}{p-1} \cdot \|f-g\|_p <\epsilon$. In the first inequality, we applied reverse triangle inequality.

Suppose that $f,g$ are in $L_1(\nu)$ with $\|f-g\|_1<\epsilon^2$. Then one has
\begin{align*}
& \nu(\left|f^{\ast}-g^{\ast}\right|>\epsilon) \leq \nu(\left|f-g\right|^{\ast})>\epsilon)= \lim_m  \nu(\sup_{n\leq m} \mathbb{E}[\left| f-g\right|\mid \mathscr{F}_n] >\epsilon) \\
\leq & \lim_m \epsilon^{-1} \cdot \mathbb{E}_{\nu} \mathbb{E}_{\nu}[\left|f-g\right|\mid \mathscr{F}_m]\leq \epsilon^{-1} \cdot \mathbb{E}_{\nu} \left|f-g\right|  \leq  \epsilon^{-1} \epsilon^{2} =\epsilon 
\end{align*}
In the first step of the first line, we apply reverse triangle inequality. The first step of the second line follows from Doob's Submartingale Inequality,\footnote{\cite[137-138]{Williams1991aa}.} where we apply it to the martingale $\mathbb{E}[\left| f-g\right|\mid \mathscr{F}_n]$. 
\end{proof}


==> 15.5-statistics.tex <==
\section{Bayesian refined lines and statistical inference}\label{sec:statistics}

The next example comes from statistics, and so we state it using that terminology and notation.\footnote{See e.g. \cite[232]{Shao2008-rf}, whose notation we follow.} A basic object in Bayesian statistical inference is a family of probability measures  $\{\mathbb{P}_{\theta}: \theta\in \Theta\}$ on the sample space~$\mathcal{X}$ indexed by elements of the parameter space $\Theta$. The following proposition shows that if one puts effectivity constraints on the two spaces $\Theta, \mathcal{X}$ as well as on the function $\theta\mapsto \mathbb{P}_{\theta}$, then this function is one component of the disintegration of a very natural $\sigma$-algebra. Namely, the $\sigma$-algebra $\mathscr{F}$ on $\Theta\times \mathcal{X}$ which contains all information about the parameter space $\Theta$ and contains no information about the sample space $\mathcal{X}$.
\begin{prop}\label{prop:bayesianprior:2} (Bayesian parameter space and sample space). Suppose that $\Theta$ (the parameter space) and $\mathcal{X}$ (the sample space) are computable Polish spaces. Suppose that $\Pi$ (the prior) is a computable probability measure on $\Theta$. Suppose that $\{\mathbb{P}_{\theta}: \theta\in \Theta\}$ is a family of probability measures on the sample space $\mathcal{X}$ such that the map $\theta\mapsto \mathbb{P}_{\theta}(V)$ is uniformly lsc for c.e. open $V\subseteq \mathcal{X}$.

Define a computable probability measure on $\Theta\times \mathcal{X}$ (the joint distribution) by $P(A)=\int_\Theta \mathbb{P}_{\theta}(A_{\theta}) \; d\Pi(\theta)$ for Borel $A\subseteq \Theta\times \mathcal{X}$, so that for $B\subseteq \Theta$ and $C\subseteq \mathcal{X}$ one has 
\begin{equation}\label{eqn:bayesianprior0v2}
P(B\times C) = \int_B \mathbb{P}_{\theta}(C)\; d\Pi(\theta)
\end{equation}

Let $\mathscr{F}$ be the effective $\sigma$-algebra on $\Theta\times \mathcal{X}$ given by sets of the form $U\times \mathcal{X}$ where $U$ ranges over a $\Pi$-computable basis on $\Theta$. 

Then the map $\rho$ from $\Theta\times \mathcal{X}$ to probability measures on $\Theta\times \mathcal{X}$ given by $\rho_{(\theta,x)} = \delta_{\theta}\otimes \mathbb{P}_{\theta}$ is a Kurtz disintegration of $\mathscr{F}$ with respect to $P$, and one has the following expression for the version of conditional expectation:
\begin{equation}\label{eqn:bayesianprior:2}
\mathbb{E}_{P}[f\mid \mathscr{F}](\theta,v) = \int_\mathcal{X} \; f(\theta,x) \; d\mathbb{P}_{\theta}(x)
\end{equation}
\end{prop}

To prove the previous proposition, we first restate it in our familiar notation and terminology, so as to better emphasise the similarity of methods and ideas with the previous proofs:
\begin{prop}\label{prop:bayesianprior} Suppose that $Y,Z$ are computable Polish spaces. Suppose that $\lambda$ is a computable point of $\mathcal{P}(Y)$. Suppose that $\mu_{\cdot}:Y\rightarrow \mathcal{P}(Z)$ is such that the map $u\mapsto \mu_u(V)$ from $Y$ to $[0,\infty)$ is uniformly lsc for c.e. open $V\subseteq Z$. 

Define a computable point $\nu$ of $\mathcal{P}(Y\times Z)$ by $\nu(A)=\int_Y \mu_u(A_u) \; d\lambda(u)$ for Borel $A\subseteq Y\times Z$, so that for $B\subseteq Y$ and $C\subseteq Z$ one has 
\begin{equation}\label{eqn:bayesianprior0}
\nu(B\times C) = \int_B \mu_u(C)\; d\lambda(u)
\end{equation}

Let $\mathscr{F}$ be the effective $\sigma$-algebra on $Y\times Z$ given by sets of the form $U\times Z$ where $U$ ranges over a $\lambda$-computable basis on $Y$. 

Then the map $\rho:Y\times Z\rightarrow \mathcal{P}(Y\times Z)$ given by $\rho_{(u,v)} = \delta_u\otimes \mu_u$ is a Kurtz disintegration of $\mathscr{F}$ with respect to $\nu$, and one has the following expression for the version of conditional expectation:
\begin{equation}\label{eqn:bayesianprior}
\mathbb{E}_{\nu}[f\mid \mathscr{F}](u,v) = \int_Z \; f(u,t) \; d\mu_u(t)
\end{equation}
\end{prop}

\begin{proof}
First note that $\nu$ is in $\mathcal{P}(Y\times Z)$, since we have:
\begin{itemize}[leftmargin=*]
\item $\mu_u((Y\times Z)_u)=\mu_u(Z)=1$, and so $\nu(Y\times Z) = \int_Y 1 \; d\lambda(u) = 1$.
\item $\mu_u((\bigsqcup_i A_i)_u) = \sum_i \mu_u((A_i)_u)$, and so $\nu(\bigsqcup_i A_i) = \int_Z \sum_i \mu_u((A_i)_v) \; d\lambda(u) = \sum_i \int_Z \mu_u((A_i)_u) \; d\lambda(u) = \sum_i \nu(A_i)$.
\end{itemize}
Second, note that $\nu$ is a computable point of $\mathcal{P}(Y\times Z)$:
\begin{itemize}[leftmargin=*]
\item It suffices by Proposition~\ref{prop:hoyruprojas} to show that $\nu(W)$ is left-c.e. as $W$ ranges over c.e. opens $W \subseteq X\times Y$.
\item For a c.e. open $W\subseteq X\times Y$, we can write it as $W=\bigcup_i U_i\times V_i$, where $U_i\subseteq U_{i+1}$ is a computable sequence of c.e. opens in $Y$ and $V_i\subseteq V_{i+1}$ is a computable sequence of c.e. opens in $Z$.
\item Note that the function $u\mapsto  I_{U_i}(u)\cdot \mu_u(V_i)$ from $Y$ to $[0,1]$ is lsc since for rational $q\geq 0$ one has $I_{U_i}(u)\cdot \mu_u(V_i)>q$ which happens iff $u$ in $U_i$ and $\mu_u(V_i)>q$, and the latter is a c.e. open condition in variable $u$ by hypothesis of the proposition.
\item Further, note that for $u$ in $Y$ we have $\mu_u((U_i\times V_i)_u) = I_{U_i}(u)\cdot \mu_u(V_i)$, since if $u$ in $U_i$ then $(U_i\times V_i)_u = V_i$, while if $u$ is not in $U_i$, then $(U_i\times V_i)_u$ is empty.
\item Then $\nu(W)>q$ iff there is $i\geq 0$ such that $\nu(U_i\times V_i)>q$, which happens iff $\int_Y I_{U_i}(u)\cdot \mu_u(V_i) \; d\lambda(u)>q$, which is a c.e. condition due to this being the expectation of the non-negative lsc function $u\mapsto I_{U_i}(u)\cdot \mu_u(V_i)$ (cf. Proposition~\ref{prop:exptoflsc}).
\end{itemize}
Third, note that for $f$ in $L_1(\nu)$, one has 
\begin{equation}\label{eqn:bayesianprior:1}
\int_{Y\times Z} f(u,v) \; d\nu(u,v) = \int_Y \int_Z \; f(u,v) \; d\mu_u(v) \; d\lambda(u)
\end{equation}
\begin{itemize}[leftmargin=*]
\item This is an induction. We just note the base case. For a Borel event $B\subseteq Y\times Z$, we have $\int_{Y\times Z} \; I_B(u,v) \; d\nu(u,v) = \nu(B) = \int_Y \mu_u(B_u) \; d\lambda(u) = \int_Y \int_Z I_{B}(u,v) \; d\mu_u(v) \; d\lambda(u)$.
\end{itemize}


Fourth, note that for any $f$ in $L_1(\nu)$, we have the following by Fubini-Tonelli:
\begin{equation*}
\mathbb{E}_{\nu}[f\mid \mathscr{F}](u,v) = \int_{Y\times Z} \; f(s,t)\; d_{\rho(u,v)}(s,t) = \int_Z \int_Y f(s,t)\; d\delta_u(s) \; d\mu_u(t) = \int_Z f(u,t) \; d\mu_u(t)
\end{equation*}
Since $v$ from $Z$ does not appear on the right-hand side, we can remove the middle integral to get the second identity:
\begin{align*}
& \int_{B\times Z}  \mathbb{E}_{\nu}[f\mid \mathscr{F}](u,v) \; d\nu(u,v) = \int_B \int_Z \; \int_Z f(u,t) \; d\mu_u(t) \; d\mu_u(v) \; d\lambda(u) \\
=&  \int_B  \int_Z f(u,t) \;  d\mu_u(t) \; d\lambda(u) = \int_{B\times Z} f(u,v) \; d\nu(u,v)
\end{align*}
In this, the first and last identities follow from two applications of the third point above. Since this holds for all Borel $B\subseteq Y$ we have that (\ref{eqn:bayesianprior}) is a version of the conditional expectation of $f$ with respect to $\mathscr{F}$.

Suppose that $(u,v)$ in $\mathsf{KR}^{\nu}(Y\times Z)$. First we note that $u$ is in $\mathsf{KR}^{\lambda}(Y)$. Suppose that $U\subseteq Y$ is a c.e. open with $\lambda(U)=1$. Then $U\times Z$ is a c.e. open with $\nu(U\times Z)=\int_U \mu_u ((U\times Z)_u) \; d\lambda(u) = \int_Y I_{U}(u)\cdot  \mu_u(Z)\; d\lambda(u) = \lambda(U)=1$. Hence $(u,v)$ is in $U\times Z$, and thus $u$ is in $U$. 

Second, suppose that $(u,v)$ in $\mathsf{KR}^{\nu}(Y\times Z)$; we want to show that $\rho_{(u,v)}([(u,v)]_{\mathscr{F}}\cap \mathsf{KR}^{\nu}(Y\times Z))=1$. Since $[(u,v)]_{\mathscr{F}}=\{u\}\times Z$, this is the same as $(\delta_u\otimes \mu_u)((\{u\}\times Z) \cap \mathsf{KR}^{\nu}(Y\times Z))=1$. Let $W\subseteq Y\times Z$ be a c.e. open with $\nu(W)=1$. It suffices to show $(\delta_u\otimes \mu_u)((\{u\}\times Z) \cap W)=1$. Let $W=\bigcup_s U_s\times V_s$ where $U_s\subseteq U_{s+1}$ and $V_s\subseteq V_{s+1}$ are computable sequences of c.e. opens in $Y,Z$ respectively. Then $(\delta_u\otimes \mu_u)((\{u\}\times Z) \cap W)=1$ iff for all $\epsilon$ in $\mathbb{Q}\cap (0,1)$ there is $s\geq 0$ such that $(\delta_u\otimes \mu_u)((\{u\}\times Z)  \cap (U_s\times V_s))>1-\epsilon$, which happens iff $\delta_u(U_s)\cdot \mu_u(V_s)>1-\epsilon$, which happens iff both $u$ in $U_s$ and $\mu_u(V_s)>1-\epsilon$.

To show this, first note that since $\nu(W)=1$, we have by our earlier calculations that $\lim_s \int_Y I_{U_s}(u)\cdot \mu_u(V_s) \; d\lambda(u)=1$. Let $g_s(u)=I_{U_s}(u)\cdot \mu_u(V_s)$, so that $0\leq g_s\leq g_{s+1}\leq 1$ is a computable sequence of lsc functions with $\mathbb{E}_{\lambda} g_s \rightarrow 1$. Hence $g_s\rightarrow 1$ in $L_1(\lambda)$, and hence $g_s\rightarrow 1$ in $L_0(\lambda)$. Let $\epsilon$ in $\mathbb{Q}\cap (0,1)$. Then $\lim_s \lambda(\left|g_s-1\right|\geq \epsilon)=0$. Since $0\leq g_s\leq 1$, this means that $\lim_s \lambda(1-\epsilon \geq g_s)=0$ and hence  $\lim_s \lambda(1-\epsilon < g_s)=1$. Since $g_s$ is non-decreasing, the set $\bigcup_s \{y\in Y: 1-\epsilon < g_s(y)\}$ is c.e. open with $\lambda$-measure one. Since $u$ is in $\mathsf{KR}^{\lambda}(Y)$ by the earlier paragraph, we have that $g_s(u)>1-\epsilon$. By definition of $g_s$, this means that both $u$ is in $U_s$ and $\mu_u(V_s)>1-\epsilon$, which is what we wanted to show.

Finally, suppose that $W\subseteq Y\times Z$ is c.e. open. As above decompose it as $W=\bigcup_s U_s\times V_s$. We want to show that $(u,v)\mapsto \rho_{(u,v)}(W)$ is uniformly lsc. For rational $q\geq 0$, we have that $\rho_{(u,v)}(W)>q$ iff there is $s\geq 0$ such that $(\delta_u\otimes \mu_u)(U_s\times V_s)>q$, which happens iff both $u$ is in $U_s$ and $\mu_u(V_s)>q$, which is clearly a c.e. open condition in variables $(u,v)$.

\end{proof}

% \begin{Q}
% Is the above example an example of a Schnorr or Martin-L\"of disintegration?

% As a concrete case, let $Y$ be the unit interval $[0,1]$ and let $\lambda$ be Lebesgue measure on $Y$, and let $Z$ be Cantor space $2^{\mathbb{N}}$, and let $\mu_p$ be the ``unfair'' coin measure on $Z$ with bias $p$. Then the joint distribution $\nu$ on $Y\times Z$ is given by $\nu((a,b)\times [\sigma])=\int_a^b p^{\#\sigma}\cdot (1-p)^{\left|\sigma\right|-\#\sigma} \; d\lambda(p)$, where $\#\sigma = \{i<\left|\sigma\right|: \sigma(i)=1\}$.

% Is it the case that if $(p,\omega)$ is in $\mathsf{SR}^{\nu}(Y\times Z)$, then $\mu_p(\{\omega^{\prime}\in 2^{\mathbb{N}} : (p,\omega^{\prime}) \in \mathsf{SR}^{\nu}(Y\times Z)\})=1$? And similarly for $\mathsf{MLR}^{\nu}(Y\times Z)$?
% \end{Q}


==> 19-ed-levy.tex <==

\section{L\'evy's Theorem for Effective Disintegrations}\label{sec:ed-levy}

\begin{cor}
Suppose that $\nu$ is a computable point of $\mathcal{P}(X)$. Suppose that $\mathscr{F}_n$ is an almost-full effective refined partition.  Define the function $\mathbb{E}_{\nu}[\cdot \mid \mathscr{F}_n](\cdot): \mathbb{L}_p^+(\nu)\times X\rightarrow [0,\infty)$ by
\begin{equation}\label{eqn:cor:main:levy:rederive}
\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x) = \sum_{\sigma\in I_n^+} \bigg(\frac{1}{\nu(U_{\sigma})} \int_{U_{\sigma}} f \; d\nu\bigg) \cdot I_{U_{\sigma}}(x)
\end{equation}
Then for all computable $p\geq 1$, the following are equivalent for $x$ in $X$: 
  \begin{itemize}[leftmargin=*]
  \item  $x$ is in $\mathsf{SR}^{\nu}$.
  \item  $x$ is in $\mathsf{KR}^{\nu}$ and $f(x)=\lim_n \mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)$ for every $L_p(\nu)$ Schnorr test $f$.
  \item  $x$ is in $\mathsf{KR}^{\nu}$ and $\lim_n \mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)$ exists for every $L_p(\nu)$ Schnorr test $f$.
  \item  $x$ is in $\mathsf{KR}^{\nu}$ and $f_{\infty}(x)=\lim_n \mathbb{E}_{\nu}[f \mid \mathscr{F}_n](x)$ for every $L_p(\nu)$ computable $f$ with witness $f_m$.  
  \item  $x$ is in $\mathsf{KR}^{\nu}$ and $\lim_n \mathbb{E}_{\nu}[f \mid \mathscr{F}_n](x)$ exists for every $L_p(\nu)$ computable $f$ with witness $f_m$.    
\end{itemize}
\end{cor}
\begin{proof}
This is by the previous Theorem and Proposition~\ref{prop:partitionsaredisintegrations}. Note that in the fourth and fifth items, we have replaced $\mathbb{E}_{\nu}[f_{\infty} \mid \mathscr{F}_n]$ with $\mathbb{E}_{\nu}[f \mid \mathscr{F}_n]$. This is justified since $f_{\infty}$ is a version of $f$, and as one can see from (\ref{eqn:cor:main:levy:rederive}), the value of $\mathbb{E}_{\nu}[f_{\infty}\mid \mathscr{F}_n]$ is equal everywhere to $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n]$, since the functions $f,f_{\infty}$ are occurring therein entirely under the integral signs. 
\end{proof}

Here is the convergence to the truth result for the combination of lines and refined partitions:
\begin{cor}


Suppose that $Y,Z$ are computable Polish spaces. Suppose that $\lambda$ is a computable point of $\mathcal{P}(Y)$ and $\mu$ is a computable point of $\mathcal{P}(Z)$. 

Suppose that $\mathscr{F}_n$ is a full effective partition of $Z$ (resp. almost-full).

Let $\mathscr{G}_n$ be the full effective filtration  $\{U\times A: U\subseteq Y \mbox{ c.e. open } \; \& \; A\in \mathscr{F}_n\}$ of $X\times Z$ (resp. almost-full).

Let $p>1$ be computable. 

Define the function $\mathbb{E}_{\lambda \otimes \mu}[\cdot \mid \mathscr{G}_n](\cdot): \mathbb{L}_p^+(\lambda\otimes \mu)\times Y\times Z \rightarrow [0,\infty]$ by
\begin{equation*}
\mathbb{E}_{\lambda\otimes\mu} [f \mid \mathscr{G}_n](u,v)= \sum_{i\in I_n^+} \bigg(\frac{1}{\mu(V_i)} \int_{V_i} f(u,t) \; d\mu(t)\bigg) \cdot I_{V_i}(v)
\end{equation*}

Then the following are equivalent for $(u,v)$ in $Y\times Z$: 
  \begin{itemize}[leftmargin=*]
  \item  $(u,v)$ is in $\mathsf{SR}^{\lambda\otimes \mu}(Y\times Z)$.
  \item  $(u,v)$ is in $\mathsf{KR}^{\lambda\otimes \mu}(Y\times Z)$ and $f(u,v)=\lim_n \mathbb{E}_{\lambda\otimes \mu}[f\mid \mathscr{G}_n](u,v)$ for every $L_p(\lambda\otimes \mu)$ Schnorr test $f:Y\times Z\rightarrow [0,\infty]$.
  \item  $(u,v)$ is in $\mathsf{KR}^{\lambda\otimes \mu}(Y\times Z)$ and $\lim_n \mathbb{E}_{\lambda\otimes \mu}[f\mid \mathscr{G}_n](u,v)$ exists for every $L_p(\lambda\otimes \mu)$ Schnorr test $f:Y\times Z\rightarrow [0,\infty]$
   \item  $(u,v)$ is in $\mathsf{KR}^{\lambda\otimes \mu}(Y\times Z)$ and $f_{\infty}(u,v)=\lim_n \mathbb{E}_{\lambda\otimes \mu}[f_{\infty}\mid \mathscr{G}_n](u,v)$ for every $L_p(\lambda\otimes \mu)$ computable $f$ with witness $f_m$.
   \item  $(u,v)$ is in $\mathsf{KR}^{\lambda\otimes \mu}(Y\times Z)$ and $\lim_n \mathbb{E}_{\lambda\otimes \mu}[f_{\infty}\mid \mathscr{G}_n](u,v)$ exists for every $L_p(\lambda\otimes \mu)$ computable $f$ with witness $f_m$.
\end{itemize}

If $p=1$, then $(u,v)$ being in $\mathsf{MLR}^{\lambda\otimes\nu}(Y\times Z)$ entails the second item in the list.

\end{cor}
\begin{proof}
This is by the previous theorem and Proposition~\ref{prop:combinepartitionslines1} and Example~\ref{ex:combinepartitionslines2}.
\end{proof}

This is the convergence to the truth result for lines from countable products:
\begin{cor}
Let $X=\prod X_i$, where $X_i$ is a computable sequence of computable Polish spaces. Let a computable point $\nu$ of $\mathcal{P}(X)$ be given by $\nu=\bigotimes_i \nu_i$, where $\nu_i$ is a computable sequence in $\mathcal{P}(X_i)$. Let $n\geq 1$. Let $\mathscr{F}_n$ be the $\sigma$-algebra on $X$ generated by sets of the form $\prod_{i\leq n} V_i\times \prod_{i>n} X_i$, where $V_i$ for $i\leq n$ ranges over c.e. opens from a $\nu_i$-computable basis on $X_i$. 

Let $p>1$ be computable. 

Define the function $\mathbb{E}_{\nu}[\cdot \mid \mathscr{F}_n](\cdot): \mathbb{L}_p^+(\nu)\times X \rightarrow [0,\infty]$ by
\begin{equation*}
\mathbb{E}_{\nu} [f \mid \mathscr{F}_n](x_1, \ldots, x_n, x_{n+1}, x_{n+2}, \ldots)=\int_{\prod_{i>n} X_i} f(x_1, \ldots, x_n, t_{n+1}, t_{n+2}, \ldots) \; d(\otimes_{i>n} \nu_i)(t_{n+1}, t_{n+2}, \ldots)
\end{equation*}
Then the following are equivalent for $x$ in $X$: 
  \begin{itemize}[leftmargin=*]
  \item  $x$ is in $\mathsf{SR}^{\nu}$.
  \item  $x$ is in $\mathsf{KR}^{\nu}$ and $f(x)=\lim_n \mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)$ for every $L_p(\nu)$ Schnorr test $f$.
  \item  $x$ is in $\mathsf{KR}^{\nu}$ and $\lim_n \mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)$ exists for every $L_p(\nu)$ Schnorr test $f$
    \item  $x$ is in $\mathsf{KR}^{\nu}$ and $f_{\infty}(x)=\lim_n \mathbb{E}_{\nu}[f_{\infty} \mid \mathscr{F}_n](x)$ for every $L_p(\nu)$ computable $f$ with witness $f_m$.
    \item  $x$ is in $\mathsf{KR}^{\nu}$ and $\lim_n \mathbb{E}_{\nu}[f_{\infty} \mid \mathscr{F}_n](x)$ exists for every $L_p(\nu)$ computable $f$ with witness $f_m$.    
\end{itemize}

If $p=1$, then $x$ being in $\mathsf{MLR}^{\nu}(X)$ entails the second item in the list.
\end{cor}

\begin{proof}
This is by the previous theorem and Example~\ref{ex:linescountableproduct} and Example~\ref{ex:linescountableproduct2}.
\end{proof}



==> 23-rates.tex <==
\section{Computable modului of convergence}\label{sec:rates}

Recall that relative to the hypotheses of Theorem~\ref{thm:newnewlevy}, we had asked the following question:

\qrates*
\noindent (Recall that the notion of computable modulus of convergence was defined in Definition~\ref{defn:core}(\ref{defn:core:16})).

In this brief section, we discuss what is known about this question in the simple setting where $X$ is Cantor space and $\nu$ is the uniform measure and with $\mathscr{F}_n$ the full effective refined partition of clopens of length $n$. In this setting, the simplest case is that of $p=1$ and $f=I_U$ where $U$ is c.e. open with $0<\nu(U)<1$ computable. In this case, the question is:

\begin{Q}\label{qratescantor}
For all $\omega$ in~$\mathsf{SR}^{\nu}$ of hyperimmune degree, and all $U$ c.e. open with $0<\nu(U)<1$ computable, is there a computable modulus for the convergence $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$? 
\end{Q}
\noindent Note that the interesting case is when $\omega\notin U$, so that the convergence in question is $\nu(U\mid [\omega\upharpoonright n])\rightarrow 0$.

In this short section we note answers to various special cases and modifications:
\begin{itemize}[leftmargin=*]
\item The question has a positive answer if one additionally assumes $\overline{U}$ is effectively closed with $\nu(\overline{U})=\nu(U)$ (Proposition \ref{prop:rates:0}).
\item The question has a negative answer if one replaces  $\omega$ being in $\mathsf{SR}^{\nu}$ with the bare convergence $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$ (Proposition~\ref{prop:rates:1}).
\item The question has a negative answer if one removes the constraint that $\nu(U)$ is computable (Proposition~\ref{prop:rates:2}).
\item The question has a negative answer if one requires that there be a computable sequence of moduli that works for all of the Schnorr randoms and c.e. opens with computable measure (Proposition \ref{prop:rates:3}).
\item The question has a negative answer if one requires that there are finitely many computable moduli that work for measure one many of the Schnorr randoms (\ref{prop:rates:4}).
\end{itemize}


We begin with the special case where the topology of the c.e. open interacts particularly well with the measure. In this, recall that we use $\overline{\;\cdot\;}$ for topological closure. 
\begin{prop}\label{prop:rates:0}
For all $U$ c.e. open with $0<\nu(U)<1$ and $\overline{U}$ effectively closed with $\nu(\overline{U})=\nu(U)$, and all  $\omega$ in $\mathsf{KR}^{\nu}$, there is a computable modulus for the convergence $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$.
\end{prop}
\begin{proof}
Under these hypotheses, one has that $\overline{U}\setminus U$ is an effectively closed $\nu$-null set. Hence any $\omega$ in $\mathsf{KR}^{\nu}$ is either in $U$ or $X\setminus \overline{U}$. Hence, either (1) there is $n_0\geq 0$ such that for all $n\geq n_0$ one has $[\omega\upharpoonright n]\subseteq U$, so that $\nu(U\mid [\omega\upharpoonright n])=1$, or (2) there is $n_0\geq 0$ such that for all $n\geq n_0$ one has $[\omega\upharpoonright n]\subseteq X\setminus \overline{U}$, so that $\nu(X\setminus \overline{U} \mid [\omega\upharpoonright n])=1$, which implies $\nu(U\mid [\omega\upharpoonright n])=\nu(\overline{U}\mid [\omega\upharpoonright n])=0$. Hence in either case, the constant function $m:\mathbb{Q}^{>0}\rightarrow \mathbb{N}$ which returns $n_0$ is a computable modulus of convergence.
\end{proof}
\noindent Note that Proposition~\ref{prop:rates:0} makes salient dense c.e. opens $U$ with $0<\nu(U)<1$, such as in Example~\ref{ex:ceopencenzer}. The proofs in the remainder of this section thus revolve around these kinds of c.e. opens.  

In general, testing for convergence to the truth is difficult by the measures of complexity from descriptive set theory, as the following result indicates. This result is an alternative presentation of Andretta and Camerlo's work on the Lebesgue Density Theorem, at least when restricted to consideration of open sets:\footnote{\cite[Theorem 1.3]{Andretta2013-wz}. See \cite{Carotenuto2016-rt} for an effectivization when $\nu(U)$ is computable.}
\begin{thm}\label{thm:andrettacamerlo} (Andretta-Camerlo)
Suppose $U$ is dense open with $0<\nu(U)<1$. Define $U_{\infty}=\{\omega: \lim_n \left|\nu(U\mid [\omega\upharpoonright n])-I_U(\omega)\right|=0\}$. Then $U_{\infty}$ is  $\utilde{\Pi}^0_3$-complete.
\end{thm}
\begin{proof}
Let $C=X\setminus U$. Then by considering whether $\omega$ is in $U$ or $C$, we get the first line in the following, and where the second line follows from $U$ being open and $C$ being closed:
\begin{align}
U_{\infty}  & =  \{\omega\in U: \lim_n \nu(U\mid [\omega\upharpoonright n])=1\}\sqcup \{\omega\in C: \lim_n \nu(C\mid [\omega\upharpoonright n])=1\}  \notag \\
& = U \cup \{\omega: \lim_n \nu(C\mid [\omega\upharpoonright n])=1\} \label{eqn:andretta}
\end{align}
In the notation of Andretta-Camerlo, this is written as $U \sqcup \Phi(C)$. Since $U$ is dense with $0<\nu(U)<1$, the set $C$ has empty interior and positive $\nu$-measure and hence its subset $\Phi(C)$ likewise has empty interior and positive $\nu$-measure (the latter by the Lebesgue Density Theorem). Hence, by Andretta-Camerlo, the set $\Phi(C)$ is $\utilde{\Pi}^0_3$-complete. By adding it to the disjoint $\utilde{\Sigma}^0_1$ set $U$, we get $U_{\infty}$ and we continue to be $\utilde{\Pi}^0_3$-complete.\footnote{By Borel determinacy, for $n\geq 1$, $\utilde{\Pi}^0_n$-completeness in zero-dimensional Polish spaces is equivalent to being in $\utilde{\Pi}^0_n\setminus \utilde{\Sigma}^0_n$. See \cite[Theorem 22.10 p. 169]{Kechris1995}.}
\end{proof}

This implies that the variant of Question~\ref{qratescantor} which does not restrict to  $\mathsf{SR}^{\nu}$ has a negative answer:
\begin{prop}\label{prop:rates:1}
Let $U$ be dense c.e. open with $0<\nu(U)<1$. Then it is not the case that for all $\omega$ in Cantor space, one has $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$ iff it does so with a computable modulus of convergence.
\end{prop}
\begin{proof}
Suppose not. Let $m_0, m_1, \ldots$ enumerate the computable moduli such that $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$ with modulus $m_i$ for some $\omega$ in Cantor space. Then define the following sequences of closed sets:
\begin{align*}
C_i & = \{\omega : \forall \; \epsilon\in \mathbb{Q}\cap (0,1) \; \forall \; n\geq m_i(\epsilon) \; \nu(C\mid  [\omega\upharpoonright n])\geq 1-\epsilon\}
\end{align*}
By equation (\ref{eqn:andretta}) from the previous proof, one has that $U_{\infty} = \bigcup_i  (U \sqcup C_i)$, which is a $\utilde{\Sigma}^0_2$ set, contradicting the previous theorem. 
\end{proof}


\begin{prop}\label{prop:rates:5}
For any $\omega$ in $\mathsf{DR}^{\nu}$ there is dense c.e. open $U$ with $0<\nu(U)<1$ such that $\omega$ is not in $U$ and the convergence $\nu(U\mid [\omega\upharpoonright n])\rightarrow 0$ does not have a computable modulus.
\end{prop}
\begin{proof}
Suppose not. Let $k\geq 0$. Let $K$ be the halting set $\{e: \varphi_e(e)\ddownarrow\}$. Enumerate it as $e_0, e_1, \ldots$, where the map $n\mapsto e_n$ is injective.

Define $c_0=0$ and $c_{n+1}=\max(\varphi_{e_n}(e_n), c_n)+1$. 

For $k,n\geq 0$, define clopen $U_{k,n}=\{\omega: \forall \; i\in [c_{n+1}, c_{n+1}+e_n+k+1) \; \omega(i)=0\}$ and define the c.e. open $U_k=\bigcup_n U_{k,n}$. Then one has $\nu(U_{k,n})=2^{-(e_n+k+1)}$. Then $0<\nu(U)\leq \sum_n \nu(U_n)<2^{-k}$. Further, by construction $U_k$ is dense. Since $U_{k,n}$ just makes decisions on bits $\geq c_{n+1}$, it is independent of all bits $<c_{n+1}$ (since $\nu$ is uniform measure). We then have that $\nu(U_{k,n}\mid [\omega\upharpoonright c_{n+1}])=2^{-(e_n+k+1)}$ for any $\omega$, and hence $\nu(U_k\mid [\omega\upharpoonright c_{n+1}])\geq 2^{-(e_n+k+1)}$ for any $\omega$.

Let $\omega$ in $\mathsf{DR}^{\nu}$. Since $\sum_k I_{U_k}$ is an $L_1(\nu)$ Martin-L\"of test, one has that there is $k$ such that $\omega$ is not in $U_k$. Hence one has $\nu(U_k\mid [\omega\upharpoonright n])\rightarrow 0$. Suppose that $\nu(U_k\mid [\omega\upharpoonright n])\rightarrow 0$ with computable modulus $m$. Let $e_n$ be such that $\varphi_{e_n}(i) = m(2^{-(i+k+1)})$ for all $i\geq 0$. Then $\varphi_{e_n}(e_n)=m(2^{-(e_n+k+1)})$. Since $c_{n+1}\geq \varphi_{e_n}(e_n) =  m(2^{-(e_n+k+1)})$, 
one has that $\nu(U\mid [\omega\upharpoonright c_{n+1}])<2^{-(e_n+k+1)}$, a contradiction to the previous paragraph. 
\end{proof}



If one changes Question~\ref{qratescantor} so that one no longer requires $\nu(U)$ to be computable, then it also has a negative answer:
\begin{prop}\label{prop:rates:2v3}
There is dense c.e. open $U$ with $0<\nu(U)<1$ such that for any $\nu$-measure one set $\mathsf{XR}^{\nu}$ and any $\omega$ in $\mathsf{XR}^{\nu}\setminus U$ with $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$, this convergence does not have a computable modulus. 
\end{prop}
\begin{proof}
Suppose not. Let $K$ be the halting set $\{e: \varphi_e(e)\ddownarrow\}$. Enumerate it as $e_0, e_1, \ldots$, where the map $n\mapsto e_n$ is injective.

Define $c_0=0$ and $c_{n+1}=\max(\varphi_{e_n}(e_n), c_n)+1$. 

For each $n\geq 0$, define the clopen $U_n=\{\omega: \forall \; i\in [c_{n+1}, c_{n+1}+e_n+1) \; \omega(i)=0\}$ and define the c.e. open $U=\bigcup_n U_n$. Then one has $\nu(U_n)=2^{-(e_n+1)}$. Since $n\mapsto e_n$ is injective but not surjective, we have $0<\nu(U)\leq \sum_n \nu(U_n)<1$. Further, by construction $U$ is dense. Since $U_n$ just makes decisions on bits $\geq c_{n+1}$, it is independent of all bits $<c_{n+1}$ (since $\nu$ is uniform measure). We then have that $\nu(U_n\mid [\omega\upharpoonright c_{n+1}])=2^{-(e_n+1)}$ for any $\omega$, and hence $\nu(U\mid [\omega\upharpoonright c_{n+1}])\geq 2^{-(e_n+1)}$ for any $\omega$.

Let $\omega$ in $\mathsf{XR}^{\nu}$ not in $U$ such that 
$\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$. (These points exist by $0<\nu(U)<1$ and the Lebesgue Density Theorem). Suppose that $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$ with computable modulus $m$. Let $e_n$ be such that $\varphi_{e_n}(k) = m(2^{-(k+1)})$ for all $k\geq 0$. Then $\varphi_{e_n}(e_n)=m(2^{-(e_n+1)})$. Since $c_{n+1}\geq \varphi_{e_n}(e_n) =  m(2^{-(e_n+1)})$, 
one has that $\nu(U\mid [\omega\upharpoonright c_{n+1}])<2^{-(e_n+1)}$, a contradiction to the previous paragraph. 
\end{proof}

The following proposition shows that Question~\ref{qratescantor} has a negative answer if one in addition insists that the computable moduli be uniform among all the c.e. opens and Schnorr randoms:
\begin{prop}\label{prop:rates:3}
There is no uniformly computable sequence $m_i:\mathbb{Q}^{>0}\rightarrow \mathbb{N}$ such that for all c.e. open $U$ with $0<\nu(U)<1$ computable and $\omega$ in $\mathsf{SR}^{\nu}$ there is $i\geq 0$ such that $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$ with modulus $m_i$ of convergence.
\end{prop}
\begin{proof}
Suppose not. Define $c_0=0$ and $c_{n+1}=\max\{m_n(2^{-(n+1)}), b_n\}+ 1$. 

For each $n\geq 0$, define the clopen $U_n=\{\omega: \forall \; i\in [c_{n+1}, c_{n+1}+n+1) \; \omega(i)=0\}$ and define the c.e. open $U=\bigcup_n U_n$. Then as in Example~\ref{ex:ceopencenzer}, one has $\nu(U_n)=2^{-(n+1)}$ and $0<\nu(U)\leq \frac{1}{3}$ is computable and $U$ is dense. As in the previous proof, for any $\omega$, we have $\nu(U_n\mid [\omega\upharpoonright c_{n+1}])=2^{-(n+1)}$, and hence $\nu(U\mid [\omega\upharpoonright c_{n+1}])\geq 2^{-(n+1)}$.

Choose $\omega$ in $\mathsf{SR}^{\nu}$ and not in $U$. Suppose that $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$ with modulus $m_n$ of convergence. Since $c_{n+1}\geq m_n(2^{-(n+1)})$ one has $\nu(U\mid [\omega\upharpoonright c_{n+1}])<2^{-(n+1)}$, a contradiction to the previous paragraph.
\end{proof}


The following proposition shows that Question~\ref{qratescantor} has a negative answer if one loosens it to a finite list of moduli and uniformizes it by insisting that these work for $\nu$-measure one many of the Schnorr randoms:
\begin{prop}\label{prop:rates:4}
There is a c.e. open $U$ with $0<\nu(U)<1$ computable such that there is no finite sequence of computable $m_1, \ldots, m_k:\mathbb{Q}^{>0}\rightarrow \mathbb{N}$ such that for $\nu$-measure one many $\omega$ in $\mathsf{SR}^{\nu}$ there is $i\in [1,k]$ such that $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$ with modulus $m_i$ of convergence.
\end{prop}
\begin{proof}
Let $U$ be as in Example~\ref{ex:ceopencenzer}, so that $U$ is dense c.e. open with $0<\nu(U)<1$ computable. Suppose for reductio there was such a finite sequence. Let  $m=\max_{i\in [1,k]} m_i$, which is also computable. Let $\mathsf{XR}^{\nu}$ be the $\nu$-measure one subset of $\mathsf{SR}^{\nu}$ from the reductio hypothesis. Then for all $\omega$ in $\mathsf{XR}^{\nu}$ one has that $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$ with modulus $m$ of convergence. Then on $\mathsf{XR}^{\nu}$ one has the following identity:
\begin{equation*}
U = \{ \omega: \forall \; \epsilon\in \mathbb{Q}\cap (0,1) \; \nu(U\mid [\omega\upharpoonright m(\epsilon)])\geq 1-\epsilon\}
\end{equation*}
Since $\nu(U)$ and $m$ are computable, the latter is an effectively closed set. This contradicts $\nu(U)<\nu(\overline{U})$ and Proposition~\ref{prop:closureissues}(\ref{prop:closureissues:1}).
\end{proof}


% \begin{prop}\label{prop:rates}
% Let $X$ be Cantor space, and let $\nu$ be uniform measure. Let $\mathscr{F}_n$ be the full filtration generated by the length $n$ strings, equipped with the effective Martin-L\"of disintegration $\rho^{(n)}=\sum_{\left|\sigma\right|=n} \nu(\cdot \mid [\sigma])\cdot I_{[\sigma]}$, which results in the version $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](\omega) = \frac{1}{\nu([\omega\upharpoonright n])} \int_{[\omega\upharpoonright n]} f \; d\nu$.

% Then it is not the case that for every $L_1(\nu)$ Schnorr test $f$ there is a function $m:\mathbb{Q}^{>0}\rightarrow \mathbb{N}$ such that 
% \begin{enumerate}[leftmargin=*]
%     \item \label{prop:rates:1} For $\nu$-measure one many $x$ in $\mathsf{SR}^{\nu}$ and  all rational $\epsilon>0$ and all $n\geq m(\epsilon)$ one has $\left|\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)-f(x)\right|<\epsilon$.
%     \item \label{prop:rates:2} For positive $\nu$-measure many $x$ in $\mathsf{SR}^{\nu}$, the point $x$ computes the function~$m$.
% \end{enumerate}
% \end{prop}

% \begin{proof}
% Let $U$ be c.e. open with $0<\nu(U)<1$ computable and $\nu(\overline{U})=1$. Let $f=I_U$, which is an $L_1(\nu)$ Schnorr test. Suppose that there was a function $m$ as described in (\ref{prop:rates:1})-(\ref{prop:rates:2}). By (\ref{prop:rates:2}) and the Sacks-Stillwell theorem, we have that $m$ is computable. Let $\mathsf{XR}^{\nu}$ be the $\nu$-measure one subset of $\mathsf{SR}^{\nu}$ as described in (\ref{prop:rates:1}).

% Since $\nu(U\cap [\sigma])$ and $\nu([\sigma])$ are uniformly computable, for rational $\epsilon$ in $(0,1)$ one has that the index set $I_{\epsilon}=\{\sigma\in 2^{<\mathbb{N}}: \left|\sigma\right|=m(\epsilon) \; \& \; \nu(U\mid [\sigma])<1-\epsilon\}$ is uniformly c.e. Hence the set $V_{\epsilon}=\bigcup_{\sigma\in I_{\epsilon}} [\sigma]$ is uniformly c.e. open. Consider the following effectively closed set: 
% \begin{equation*}
% C =\bigcap_{\epsilon\in \mathbb{Q}\cap (0,1)} X\setminus V_{\epsilon}=\{ \omega: \forall \; \epsilon\in \mathbb{Q}\cap (0,1) \; \nu(U\mid [\omega\upharpoonright m(\epsilon)])\geq 1-\epsilon\}
% \end{equation*}

% Then we argue that $U=C$ on $\mathsf{XR}^{\nu}$:
% \begin{itemize}[leftmargin=*]
% \item Suppose that $\omega$ is in $\mathsf{XR}^{\nu}$.
% \item Suppose that $\omega$ is in $U$. Then $f(\omega)=1$. Since $\omega$ is in $\mathsf{SR}^{\nu}$ and since $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](\omega)=\nu(U\upharpoonright [\omega \upharpoonright n])$, we have by (\ref{prop:rates:2}) that $\left|\nu(U\mid [\omega\mid n])-1\right|<\epsilon$ for all $n\geq m(\epsilon)$ and all rational $\epsilon$ in the interval $(0,1)$. Then $\nu(U\mid [\omega\mid m(\epsilon)])> 1-\epsilon$ for all such $\epsilon$ and this puts $\omega$ into $C$.
% \item Suppose that $\omega$ is $C$. We want to show that $\omega$ is in $U$. Suppose not. Then $f(\omega)=0$. Since $\omega$ is in $\mathsf{SR}^{\nu}$, we have by (\ref{prop:rates:2}) that $\left|\nu(U\mid [\omega\mid n])-0\right|<\epsilon$ for all $n\geq m(\epsilon)$ and all rational $\epsilon$ in the interval $(0,1)$. For $\epsilon$ in the interval $(0,\frac{1}{2})$ this results in a contradiction to membership in $C$.
% \end{itemize}
% Hence indeed $U=C$ on $\mathsf{XR}^{\nu}$. This contradicts $\nu(U)<\nu(\overline{U})$ and Proposition~\ref{prop:closureissues}(\ref{prop:closureissues:1}).
% \end{proof}

% % 

==> extras-more.tex <==




\begin{Q}
Let $\nu$ be a computable point of $\mathcal{P}(2^{\mathbb{N}})$. 

Is there a uniformly computable sequence of c.e. opens $V_m$ such that
\begin{itemize}
\item $V_m$ has uniformly computable $\nu$-measure.
\item There is $\omega$ in $\mathsf{SR}^{\nu}$ such that $\{m: \omega\in V_m\}\nleq_T \omega$
\end{itemize}
Note that if there were such a sequence, then by duplicating entries we could create such a sequence with the further property that
\begin{itemize}
\item Each $\omega$ in Cantor space is in infinitely many of the $V_m$.
\end{itemize}

If yes, then Proposition~\ref{prop:enumerations:2} and Proposition \ref{prop:enumerations:3} imply that the $L_1(\nu)$ Schnorr test $h_e$ is such that $h_e(\omega)$ is not right-c.e.-in-$\omega$ for the $\omega$ in the third point. Hence we do not have that $\mathbb{E}_{\nu}[h_e\mid \mathscr{F}_n](\omega)\rightarrow h_e(\omega)$ at a computable rate of convergence, since this would imply that $h_e(\omega)$ is computable-in-$\omega$. (Here we are thinking about $\mathscr{F}_n$ as the natural filtration on Cantor space, generated by length $n$ strings. ).


\end{Q}






\begin{prop}\label{prop:enumerations:3}
Let $\nu$ be a computable point of $\mathcal{P}(2^{\mathbb{N}})$.

Suppose that $V_m$ is a computable sequence of c.e. opens (resp. with $\nu(V_m)$ having uniformly computable $\nu$-measure) and such that each element of Cantor space is in infinitely many of the $V_m$.

Let $e$ be a Turing program such that $W_e^{\omega}=\{m: \omega\in V_m\}$. 

Then the function $h_e:2^{\mathbb{N}}\rightarrow [0,\infty]$ as in Proposition~\ref{prop:enumerations:2} is an $L_1(\nu)$ Martin-L\"of test (resp. $L_1(\nu)$ Schnorr test).

\end{prop}
\begin{proof}
Define the following c.e. opens:
\begin{equation*}
U_{n,m} =\{\omega\in 2^{\mathbb{N}} : \exists \; s \; \left|W_{e,s+1}^{\omega}\right|=n \; \& \; m\in W_{e,s+1}^{\omega}\setminus W_{e,s}^{\omega}\}
\end{equation*}
This is also effectively closed, as one can see from:
\begin{equation*}
U_{n,m} =\{\omega\in 2^{\mathbb{N}} : \forall \; s \; \forall \; m^{\prime} \; \big(\big(\left|W_{e,s+1}^{\omega}\right|=n \; \& \; m^{\prime}\in W_{e,s+1}^{\omega}\setminus W_{e,s}^{\omega}\big) \rightarrow m=m^{\prime}\big)\}
\end{equation*}
Further, since $W_e^{\omega}$ infinite for all $\omega$ in $2^{\mathbb{N}}$, for all $n\geq 0$, we have that $2^{\mathbb{N}}=\bigsqcup_m U_{n,m}$ and further for all $m\geq 0$ we have $V_m=\bigsqcup_n U_{n,m}$. Hence one has the decomposition $h_e(\omega) = \sum_n 2^{-g_e(\omega)(n)} = \sum_n \sum_m 2^{-m}\cdot I_{U_{n,m}}$. From this we calculate the expectation as follows 
\begin{equation}\label{eqn:done}
\mathbb{E}_{\nu} h_e = \sum_n \sum_m 2^{-m}\cdot \nu(U_{n,m}) =\sum_m 2^{-m} \cdot \sum_n \nu(U_{n,m}) = \sum_m 2^{-m} \nu(V_m)
\end{equation}
Hence $h_e$ is an $L_1(\nu)$ Martin-L\"of test. And if $\nu(V_m)$ is uniformly computable, then this expectation is computable and hence $h_e$ is an $L_1(\nu)$ Schnorr test.
\end{proof}


 Here is an example showing that we cannot improve this:

\begin{prop}\label{prop:enumerations:2}
Let $g_e:2^{\mathbb{N}}\rightarrow \mathbb{N}^{\mathbb{N}}$ be as in Proposition~\ref{prop:enumerations}, with $W_e^{\omega}$ infinite for all $\omega$ in $2^{\mathbb{N}}$.

Then the function $h_e:2^{\mathbb{N}}\rightarrow [0,\infty]$ by $h_e(\omega)=\sum_n 2^{-g_e(\omega)(n)}$ is non-negative lsc. Hence, for all $\omega$ in $2^{\mathbb{N}}$, one has that $h_e(\omega)$ is left-c.e.-in-$\omega$.

Further, for all $\omega$ in $2^{\mathbb{N}}$, one has that $W_e^{\omega}$ is computable in $\omega$ iff  $h_e(\omega)$ is right-c.e.-in-$\omega$. This happens iff $h_e(\omega)$ is computable in $\omega$.
\end{prop}
\begin{proof}
It is non-negative lsc since it is the composition of the computable continuous function $g_e$ with the lsc function $f\mapsto \sum_n 2^{-f(n)}$. As such, $h_e(\omega)$ is left-c.e.-in-$\omega$. 

First suppose that $\omega$ in $2^{\mathbb{N}}$ is such that $W_e^{\omega}$ is not computable in $\omega$.  Suppose for reductio that $h_e(\omega)$ is right-c.e. in $\omega$. Then $h_e(\omega)$ is computable in $\omega$, and so decidable in $\omega$, and so the left Dedekind cut of $h_e(\omega)$ is computable in $\omega$. Let $h_{e,t}(\omega)=\sum_{m<t, m\in W_e^{\omega}} 2^{-m}$. Note that $t$ is in the range $ W_e^{\omega}$ of $g_e(\omega)$ iff $h_{e,t}(\omega) + 2^{-t}<h_{e}(\omega)$, which happens iff $h_{e,t}(\omega)+2^{-t}$ is in the left Dedekind cut of $h_e(\omega)$. By recursion on $t\geq 0$, we recursively-in-$\omega$ compute membership of $\{0, \ldots, t\}$ in the range $W_e^{\omega}$  of $g_e(\omega)$, along with the rational numbers $\{h_0(\omega), \ldots, h_t(\omega)\}$. Suppose that we have computed it up to $t$; we show how to compute it for $t+1$. If $t$ is in the range $W_e^{\omega}$  of $g_e(\omega)$, then $h_{e,t+1}(\omega)=h_{e,t}(\omega) +2^{-t}$, and if not then $h_{e,t+1}(\omega)=h_{e,t}(\omega)$. Then $t+1$ is the range of $g_e(\omega)$ iff $h_{e,t}(\omega) +2^{-t}$ is in the left Dedekind cut of $h_e(\omega)$.

Second suppose that $\omega$ in $2^{\mathbb{N}}$ is such that $W_e^{\omega}$ is computable in $\omega$. Then there is a $\omega$-computable computable function $p:\mathbb{N}\rightarrow \mathbb{N}$ that enumerates $W_e^{\omega}$ in increasing order, so that $i\leq p(i)$ for all $i\geq 0$, and hence $2^{-p(i)}\leq 2^{-i}$ for all $i\geq 0$. Then by the Comparison Test, we have that $h_e(\omega)=\sum_i 2^{-p(i)}$ is computable in $\omega$.

\end{proof}


\begin{prop}\label{prop:enumerations} (Enumerations of c.e. sets as computable continuous functions).

Suppose that $e$ is an index for a Turing program such that for all $\omega$ in $2^{\mathbb{N}}$, the c.e.-in-$\omega$ set $W_e^{\omega}$ is infinite. 

Define $f_e^{\omega}:\mathbb{N}\rightarrow \mathbb{N}$ as follows: given $n$, search for the a stage $s$ such that $W_{e,s+1}^{\omega}$ has exactly $n$ elements and $W_{e,s+1}^{\omega}\setminus W_{e,s+1}^{\omega}$ is non-empty, and return the unique element of $W_{e,s+1}^{\omega}\setminus W_{e,s+1}^{\omega}$. Then $f_e^{\omega}:\mathbb{N}\rightarrow \mathbb{N}$ is uniformly computable in $\omega$ and is an injective function with range $W_e^{\omega}$.

Define $g_e:2^{\mathbb{N}}\rightarrow \mathbb{N}^{\mathbb{N}}$ by $g_e(\omega)(n)=f^{\omega}_e(n)$. Then $g_e:2^{\mathbb{N}}\rightarrow \mathbb{N}^{\mathbb{N}}$ is computable continuous. 
\end{prop}
\begin{proof}
The function $f_e^{\omega}:\mathbb{N}\rightarrow \mathbb{N}$ is uniformly computable in $\omega$ because the use conventions dictate that $W_{e,s}^{\omega}=W_{e,s}^{\omega\upharpoonright s}$, and the membership in the finite sets $W_{e,s}^{\sigma}$ of size $<s$ is uniformly computable, and hence their cardinality is also uniformly computable. This shows that the search condition in the definition of $f_e^{\omega}(n)$ is a computable query, and the search always terminates since we presumed the sets $W_e^{\omega}$ to be infinite.

Further, the function $f_e^{\omega}:\mathbb{N}\rightarrow \mathbb{N}$ is injective and has range $W_e^{\omega}$. These two points are clear from construction.

The function $g_e:2^{\mathbb{N}}\rightarrow \mathbb{N}^{\mathbb{N}}$ is continuous computable. We show that inverse images of the basic clopens are uniformly c.e. open. For $\tau$ in $\mathbb{N}^{<\mathbb{N}}$ let $I_{\tau}$ be the c.e. index set of strings $\sigma$ in $2^{<\mathbb{N}}$ such that there is $t\geq 0$ such that for all $n<\left|\tau\right|$ there is $s<t$ such that $W_{e,s+1}^{\omega}$ has exactly $n$ elements and $\tau(n)$ is the unique element of $W_{e,s+1}^{\omega}\setminus W_{e,s}^{\omega}$. Then one has that $g_e^{-1}([\tau])=\bigcup_{\sigma \in I_{\tau}}[\sigma]$.
\end{proof}


\begin{prop}\label{prop:increasemeasure2}
Suppose that $\nu$ is a computable atomless point of $\mathcal{M}^+(X)$. Given an index for a c.e. open $U$ with computable $\nu$-measure and computable real~$a$ satisfying $\nu(U)<a\leq \nu(X)$, one can compute an index for a c.e. open $V$ such that $V\supseteq U$ and $\nu(V)=a$. 
\end{prop}
\begin{proof}
Let $B_1, B_2, \ldots$ be a $\nu$-computable basis. Since $a$ is computable, choose an increasing computable sequence of rationals $p_i>\nu(U)$ converging up to $a$. It suffices to show that there is an increasing computable sequence of c.e. opens $V_i\supseteq U$ with $p_i<\nu(V_i)<p_{i+1}$ and $\nu(V_i)$ having uniformly $\nu$-computable measure. Suppose that we have constructed $V_{i-1}$, where we set $V_{-1}=U$. Classically, since $\nu$ is atomless, there is open superset of $V_{i-1}$ whose $\nu$-measure is in the interval $(p_i, p_{i+1})$.\footnote{\cite[Vol 1 p. 56]{Bogachev2007-yt}.} Since the $\nu$-computable basis is a classical basis, we can write the superset as the union of $V_{i-1}$ and countably elements of this basis. Then we can do an unbounded search for a finite sequence $B_{k_1}, \ldots, B_{k_n}$ from the $\nu$-computable basis such that $p_i<\nu(V_{i-1}\cup B_{k_1}\cup \cdots\cup B_{k_n})<p_{i+1}$, where the union has $\nu$-computable measure by Proposition~\ref{prop:mucomputablebasis}(\ref{prop:union:mucompbasis:2.2}).
\end{proof}



The question of whether and when an $L_0(\nu)$-computable point is $L_1(\nu)$-computable is resolved by effective uniform integrability. Suppose $f_0, f_1, \ldots$ is a uniformly computable sequence of points in $L_1(\nu)$ which is bounded in $L_1(\nu)$. Then the sequence $f_0, f_1, \ldots$ is \emph{computably uniformly integrable} if there is a computable map $m:\mathbb{Q}^{>0}\rightarrow \mathbb{Q}^{>0}$ such that $\int_{\left|f_n\right|>m(\epsilon)} \left|f\right|\; d\nu<\epsilon$ for all $n\geq 0$. This is equivalent to there being a computable map $m:\mathbb{Q}^{>0}\rightarrow \mathbb{Q}^{>0}$ such that that $\nu(A)<m(\epsilon)$ implies $\int_A \left|f_n\right|\; d\nu<\epsilon$ for all events $A$ and all $n\geq 0$. 

If we take a single $L_1(\nu)$-computable $f$, then the constant sequence $f, f, f, \ldots$ is computably uniformly integrable:
\begin{ex}\label{ex:cui}
Suppose $f$ is $L^1(\nu)$-computable, with witness $g_k$, with $q_k\geq \max(g_k)$ computable and $q_k>0$. Given rational $\epsilon>0$, compute  $2^{-k}<\epsilon$ and let 
$\delta=\frac{1}{2}\cdot \frac{\epsilon}{q_k}$. Suppose $A$ is a Borel event with $\nu(A)<\delta$. Then $\int_A \left|g_k\right| \; d\nu \leq q_k\cdot \nu(A)<\frac{\epsilon}{2}$. Then $\int_A \left|f\right|\; d\nu \leq \|f-g_k\|_1 +\int_A \left|g_k\right| \; d\nu<\epsilon$.
\end{ex}

The following is the natural effective version of the characterisation of convergence in $L_1(\nu)$ in terms of convergence in $L_0(\nu)$ and uniform integrability.\footnote{\cite[131-2]{Williams1991aa}.} In the statement of the following proposition, ``the countable dense set'' in the first line is that of $L_0(\nu)$ or $L_1(\nu)$, since recall that they are the same set.
\begin{prop}
If $\nu$ is a computable point of $\mathcal{P}(X)$, then a computable point of $L_0(\nu)$ is a computable point of $L_1(\nu)$ iff it has a witnessing sequence from the countable dense set which is computably uniformly integrable. 

In more detail, suppose that $f_n$ are uniformly computable points of $L_1(\nu)$, and suppose that $f$ is point of $L_0(\nu)$.

If $f_n\rightarrow f$ at geometric rate of convergence $b\geq 2$ in $L_1(\nu)$ then $f$ is a computable point of both $L_1(\nu)$  and $L_0(\nu)$ and $f_n\rightarrow f$ at geometric rate of convergence $\sqrt{b}\geq \sqrt{2}$ in $L_0(\nu)$ and $f_n$ is computably uniformly integrable. 

Conversely, if $f_n\rightarrow f$ at geometric rate of convergence $c\geq \sqrt{2}$ in $L_0(\nu)$ and $f_n$ is computably uniformly integrable, then $f$ is a computable point of both $L_1(\nu)$  and $L_0(\nu)$ and $f_{n+6}\rightarrow f$ at geometric rate of convergence $c$ in $L_1(\nu)$.
\end{prop}

\begin{proof}
Suppose that $f_n\rightarrow f$ at geometric rate of convergence $b\geq 2$ in $L_1(\nu)$. Then $f_n\rightarrow f$ fast in $L_1(\nu)$ and so $f$ is a computable point of $L_1(\nu)$ and thus a computable point of $L_0(\nu)$. Further, by Proposition~\ref{prop:bfastprop}, $f_n\rightarrow f$ in $L_0(\nu)$ at geometric rate of convergence $\sqrt{b}\geq \sqrt{2}$. It remains to show that $f_n$ is computably uniformly integrable. Consider rational $\epsilon>0$. Compute $m$ such that $b^{-m}<\frac{\epsilon}{4}$. As in Example~\ref{ex:cui}, compute rational $\delta>0$ such that for all $n\leq m$ and all Borel events $A$ one has that $\nu(A)<\delta$ implies $\int_A \left|f_n\right|\; d\nu<\frac{\epsilon}{2}$. Let $n>m$, and let $A$ be a Borel event with $\nu(A)<\delta$. Then $\int_A \left|f_n\right| \; d\nu\leq \|f_n-f\|_1+\|f-f_m\|_1+\int_A \left|f_m\right|\; d\nu \leq 2\cdot b^{-m}+\frac{\epsilon}{2}<\epsilon$.

For the converse direction, suppose that $f_n\rightarrow f$ at geometric rate of convergence $c\geq \sqrt{3}$ in $L_0(\nu)$ and suppose that the sequence $f_m$ is computably uniformly integrable. From the latter, for each $n\geq 0$ compute $K_n\geq 0$ such that $\int_{\left|f\right|>K_n} \left|f\right| \; d\nu <c^{-n}$ and $\int_{\left|f_m\right|>K_n} \left|f_m\right| \; d\nu <c^{-n}$ for all $m,n\geq 0$. Let $\varphi_n:\mathbb{R}\rightarrow [-K_n,K_n]$ by being the identity on $[-K_n,K_n]$ and by being $-K_n$ on $(-\infty, K_n]$ and by being $K_n$ on $[K_n,\infty)$. Then note for all $m,n\geq 0$ and all reals $u,v$ we have:
\begin{equation*}
\left|\varphi_n\circ f - f\right|\leq \left|f\right| \cdot I_{\left|f\right|>K_n}, \hspace{3mm} \left|\varphi_n\circ f_m - f_m\right|\leq \left|f_m\right| \cdot I_{\left|f_m\right|>K_n}, \hspace{3mm} \left|\varphi_n(u)-\varphi_n(v)\right|\leq \left|u-v\right|
\end{equation*}
From the first two follows $\|\varphi_n\circ f - f\|_1 <c^{-n}$ and $\|\varphi_n\circ f_m - f_m\|_1 <c^{-n}$, for all $m,n\geq 0$. From the last follows, for all $n\geq 0$, that $\varphi_n \circ f_m\rightarrow \varphi_n \circ f$ in $L_0(\nu)$ at geometric rate of convergence $c\geq \sqrt{2}$ in $L_0(\nu)$. By the below Proposition~\ref{prop:bddthm}, for all $n\geq 0$, one has that $\varphi_n \circ f_{m+2}\rightarrow \varphi_n \circ f$ in $L_1(\nu)$ at geometric rate of convergence $c$ in $L_1(\nu)$, so that for all $m,n\geq 0$ one has $\|\varphi_n \circ f_{m+2} - \varphi_n \circ f\|_1\leq c^{-m}$. Then one has for $n=m+4$ the following, where the last inequality follows from the hypothesis $c\geq \sqrt{2}\geq \sqrt[4]{3}$:
\begin{equation*}
\|f_{m+6}-f\|_1 \leq \| f_{m+6}-\varphi_n\circ f_{m+6}\|_1+\|\varphi_n \circ f_{m+6} - \varphi_n \circ f\|_1+\|\varphi_n\circ f - f\|_1 <c^{-m}
\end{equation*}
\end{proof}



 (Conditional MCT). 

Suppose that $f_n, f$ are in $\mathbb{L}_1^+(\nu)$ and $0\leq f_n\leq f_{n+1}$ on $\mathsf{XR}^{\nu}$ and $\lim_n f_n=f$ on $\mathsf{XR}^{\nu}$.

Then $\lim_n \mathbb{E}_{\nu}[f_n\mid \mathscr{F}] = \mathbb{E}_{\nu}[f \mid \mathscr{F}]$ on $\mathsf{XR}^{\nu}$.
\end{prop}
\begin{proof}
Let $x$ in $\mathsf{XR}^{\nu}$. Then $\rho_x$ is in $\mathcal{P}(X)$ and $\rho_{x}([x]_{\mathscr{F}}\cap \mathsf{XR}^{\nu})=1$. By hypothesis, $0\leq f_n\leq f_{n+1}$ for $\rho_x$-a.s. many points, and likewise  $\lim_n f_n=f$ for  $\rho_x$-a.s. many points. Then by MCT applied to $\rho_x$ we have $\lim_n \mathbb{E}_{\nu}[f_n\mid \mathscr{F}](x) = \mathbb{E}_{\nu}[f \mid \mathscr{F}](x)$.
\end{proof}


\begin{prop}\label{prop:cdct} (Conditional DCT). Suppose $\rho: X\rightarrow \mathcal{M}^+(X)$ is a $\mathsf{XR}^{\nu}$ disintegration of $\mathscr{F}$.

Suppose that $f_n, f, g$ are in $\mathbb{L}_1^+(\nu)$ and $0\leq f_n\leq g$ on $\mathsf{XR}^{\nu}$ and $\lim_n f_n=f$ on $\mathsf{XR}^{\nu}$ and $\int g \; d\rho_x<\infty$ for all $x$ in $\mathsf{XR}^{\nu}$. 

Then $\lim_n \mathbb{E}_{\nu}[f_n\mid \mathscr{F}] = \mathbb{E}_{\nu}[f \mid \mathscr{F}]$ on $\mathsf{XR}^{\nu}$.
\end{prop}
\begin{proof}
Let $x$ in $\mathsf{XR}^{\nu}$. Then $\rho_x$ is in $\mathcal{P}(X)$ and $\rho_{x}([x]_{\mathscr{F}}\cap \mathsf{XR}^{\nu})=1$. By hypothesis, $0\leq f_n\leq g$ for $\rho_x$-a.s. many points, and likewise  $\lim_n f_n=f$ for  $\rho_x$-a.s. many points. Further since $x$ is in $\mathsf{XR}^{\nu}$, we have by hypothesis that $g$ is in $\mathbb{L}^+_1(\rho_x)$. Hence by the DCT applied to $\rho_x$, we have that $\lim_n \int f_n \; d\rho_x = \int f \; d\rho_x$. Hence $\lim_n \mathbb{E}_{\nu}[f_n\mid \mathscr{F}](x) = \mathbb{E}_{\nu}[f \mid \mathscr{F}](x)$.
\end{proof}

\begin{prop}\label{prop:ctowisk} (`Taking out what is known'). Suppose $\rho: X\rightarrow \mathcal{M}^+(X)$ is a $\mathsf{XR}^{\nu}$ disintegration of $\mathscr{F}$.

Suppose that $f,g$ in $\mathbb{L}_1^+(\nu)$, and suppose that $g$ is equal on $\mathsf{XR}^{\nu}$ to a $\mathscr{F}$-measurable function.

Then $\mathbb{E}_{\nu}[f\cdot g\mid \mathscr{F}]=g\cdot \mathbb{E}_{\nu}[f\mid \mathscr{F}]$ on $\mathsf{XR}^{\nu}$.
\end{prop}
\begin{proof}
By Proposition~\ref{prop:dis:2}(\ref{prop:newlevy:2a:again}), it suffices to prove it for $g$ which is itself $\mathscr{F}$-measurable. We show it by induction on complexity of $g$. 

Suppose $g=I_A$ where $A$ is $\mathscr{F}$-measurable.  If $x$ in $A$ then $[x]_{\mathscr{F}}\subseteq A$ and then $A$ is a $\rho_x$-measure one event and then it reduces to the observation that $\int_A f(v) \; d\rho_x(v)=\int f(v) \; d\rho_x(v)$. If $x$ is not in $A$ then $[x]_{\mathscr{F}}\subseteq X\setminus A$ and then $A$ is a $\rho_x$-measure zero event and then it reduces to the observation that $\int_A f(v) \; d\rho_x(v)=0$.

By Proposition~\ref{prop:dis:2}(\ref{prop:newlevy:2b:again})-(\ref{prop:newlevy:2c:again}), it extends to simple functions. By Conditional MCT (\ref{prop:cmct}) it extends to all elements of $\mathbb{L}_1^+(\nu)$.
\end{proof}

Before proving the next proposition, we recall some elementary facts about convexity:
\begin{itemize}[leftmargin=*]
\item A subset $X$ of a real vector space is \emph{convex} if for all $x_1, x_2$ in $X$ and all $0\leq t\leq 1$, one has that the point $t\cdot x_1+(1-t)\cdot x_2$ is in $X$.
\item If $X$ is a convex subset of a real vector space, then a function $f: X\rightarrow \mathbb{R}$ is \emph{convex} if for all $x_1,x_2$ in $X$ and all $0\leq t\leq 1$, one has the inequality $f(t\cdot x_1+(1-t)\cdot x_2)\leq t\cdot f(x_1)+(1-t)\cdot f(x_2)$.
\item By induction, if  $f: X\rightarrow \mathbb{R}$ is convex, then for all $n\geq 1$ and all $x_1,\ldots, x_n$ in $X$ and all $0\leq t_1, \ldots, t_n\leq 1$ with $\sum_{i=1}^n t_i=1$, one has the inequality $f(\sum_{i=1}^n t_i\cdot x_i)\leq \sum_{i=1}^n t_i\cdot f(x_i)$.
\item Likewise, if $f: X\rightarrow \mathbb{R}$ is convex and $X$ contains $0$ and $f$ satisfies $f(0)=0$, then for all $n\geq 1$ and all $x_1,\ldots, x_n$ in $X$ and all $0\leq t_1, \ldots, t_n\leq 1$ with $\sum_{i=1}^n t_i\leq 1$, one has the inequality $f(\sum_{i=1}^n t_i \cdot x_i)\leq \sum_{i=1}^n t_i \cdot f(x_i)$. For one can simply set $t_{n+1}=1-\sum_{i=1}^n t_i$ and $x_{n+1}=0$.
\end{itemize}
In the proof of the following proposition, we apply this last point to the convex function $f(x)=\left|x\right|^p$ with domain $X=\mathbb{R}$.



We then have:
\begin{prop}\label{prop:technical}
Every effective partition has an effective softening. 
\end{prop}
\begin{proof}
Since the computable sequence $A_i$ comes from the algebra generated by a $\nu$-computable basis, by Proposition~\ref{prop:krplusbasis}, there is a computable sequence of c.e. opens $V_i$ and effectively closed $C_i\supseteq V_i$ with $\nu(C_i)=\nu(A_i)$ and $V_i=A_i$ on  $\mathsf{KR}^{\nu}$. Then no elements of $\mathsf{KR}^{\nu}$ are in $C_i\setminus V_i$, since this is an effectively closed $\nu$-null set. Then define recursively the sequence of c.e. opens by $U_0=V_0$ and $U_{n+1}=V_{n+1}\setminus \bigcup_{m\leq n} C_m$. Then the $U_n$ are pairwise disjoint by construction. Further, the $U_n$ are equal to $V_n$ on $\mathsf{KR}^{\nu}$, by induction on $n\geq 0$:
\begin{itemize}[leftmargin=*]
\item This is clear for $n=0$.
\item Suppose for induction hypothesis it is true for $n\geq 0$.
\item If $x$ is in $U_{n+1}$, then it is by construction in $V_{n+1}$.
\item If $x$ is in $\mathsf{KR}^{\nu}$ and in $V_{n+1}$, then it cannot be $\bigcup_{m\leq n} C_m$, since this would put it in $C_m$ for some $m\leq n$, and hence in $V_m$ due to it being in $\mathsf{KR}^{\nu}$. But this contradicts that $V_m=A_m$ on $\mathsf{KR}^{\nu}$ and $V_{n+1}=A_{n+1}$ on $\mathsf{KR}^{\nu}$ and $A_m\cap A_{n+1}=\emptyset$.
\end{itemize}
Hence, the $U_n$ is equal to $A_n$ on $\mathsf{KR}^{\nu}$.
\end{proof}


The following isolates the natural sufficient condition for an effective refined partition to be full, and this condition is obviously met in Examples~\ref{ex:refinedpartition}-\ref{ex:refinedlines} and in examples that involve decomposing Baire space or Cantor space into its length $n$ clopens:
\begin{prop}\label{prop:effectshrinking}
Suppose that the effective refined partition $\mathscr{F}_n$, as in the previous example, satisfies the following properties:
\begin{itemize}[leftmargin=*]
\item \emph{Effectively Shrinking}: There is a computable function $\ell:\mathbb{Q}^{>0}\rightarrow \mathbb{N}$ such that for all rational $\epsilon>0$ one has that $\mathrm{diam}(A_{\sigma})<\epsilon$ for all $\sigma$ in $T$ with $\left|\sigma\right|\geq \ell(\epsilon)$.
\item \emph{Effectively non-empty}: There is a uniformly computable sequence of points $x_{\sigma}$ in $A_{\sigma}$.
\end{itemize}
Then the effective refined partition $\mathscr{F}_n$ is full.
\end{prop}
\begin{proof}
First we argue that these two conditions entail that there is a well-defined computable continuous surjection $\pi:[T]\rightarrow X$ given by $\pi(\omega)=x$ iff $\{x\}=\bigcap_n A_{\omega\upharpoonright n}$.

Suppose that $\omega$ in $[T]$ is given. By effective non-emptiness, the point $x_{\omega\upharpoonright n}$ is in $A_{\omega_n}$. By effective shrinking, the $x_{\omega\upharpoonright n}$ is a Cauchy sequence. Hence, it has a limit $x$, which is in the intersection $\bigcap_n A_{\omega\upharpoonright n}$. Likewise, by effective shrinking, it is the only element of this intersection.

 The map  $\pi:[T]\rightarrow X$ is surjective since each $\mathscr{F}_n$ is a partition. 

 By effective shrinking, the map $\pi:[T]\rightarrow X$ has a computable modulus of uniform continuity given by $m(\epsilon)=2^{-\ell(\epsilon)}$. For, suppose that $\omega,\omega^{\prime}$ in $[T]$ with $d(\omega,\omega^{\prime})<m(\epsilon)$. Then $\sigma:=\omega\upharpoonright \ell(\epsilon)=\omega^{\prime}\upharpoonright \ell(\epsilon)$. Then by definition of $\ell(\epsilon)$, we have $\mathrm{diam}(A_{\sigma})<\epsilon$. Since $\omega, \omega^{\prime}$ are both elements of this set, we have $d(\omega, \omega^{\prime})<\epsilon$.

 By effective non-emptiness, the map $\pi$ uniformly sends the countable dense set of $[T]$ to a computable point of $X$. For a natural countable dense set of $T$ is given by computing the leftmost branch $\omega_{\sigma}$ in $[T]\cap [\sigma]$, for each $\sigma$ in $T$. Then $\pi(\omega_{\sigma})$ is the limit of the uniformly computable sequence $x_{\omega_{\sigma}\upharpoonright n}$. By effective shrinking, we can compute a subsequence of the latter which converges fast to $\pi(\omega_{\sigma})$, and so the latter is computable, uniformly in $\sigma$ from $T$. 

 Hence, by Proposition~\ref{prop:suffforcont}, we have that $\pi:[T]\rightarrow X$ is continuous computable. 

 Suppose that $U\subseteq X$ is c.e. open. Then $\pi^{-1}(U)$ is c.e. open. Then there is c.e. set $S\subseteq T$ such that $\pi^{-1}(U)=\bigcup_{\sigma\in S} [T]\cap [\sigma]$. Then we claim that $U=\bigcup_{\sigma\in S} A_{\sigma}$:
\begin{itemize}[leftmargin=*]
\item Suppose that $x$ is in $U$. By surjectivity, choose $\omega$ in $[T]$ with $\pi(\omega)=x$. Then $\omega$ in $[T]\cap [\sigma]$ for some $\sigma$ in $S$. Then by definition $\pi(\omega)$ is in $A_{\sigma}$, and so $x$ is in $A_{\sigma}$.
\item Suppose that $x$ in $A_{\sigma}$ for some $\sigma$ in $S$. By surjectivity, choose $\omega$ in $[T]$ with $\pi(\omega)=x$. Then by definition of $\pi$, we have $\{x\}=\bigcap_n A_{\omega\upharpoonright n}$. Then since $\mathscr{F}_{\left|\sigma\right|}$ is a partition, we have that $\sigma$ is an initial segment of $\omega$. Then $\omega$ is in $[T]\cap [\sigma]$, which is a subset of $\pi^{-1}(U)$. Then $\pi(\omega)$ is in $U$, and so $x$ is in $U$.
\end{itemize}
\end{proof}

==> extras.tex <==

By way of motivation for the following definition, first consider the classical situation:
\begin{prop}\label{prop:beclassical}
Let $\mathscr{F}_n$ be a full filtration equipped with disintegrations $\rho^{(n)}$.
\begin{enumerate}[leftmargin=*]
    \item \label{prop:beclassical:1} Let $U_0, U_1, \ldots$ be a basis for the topology. Then the set of points $x$ such that $\rho^{(n)}_x$ is in $\mathcal{P}(X)$ and $\lim_n \rho^{(n)}_x(U_i)=\delta_x(U_i)$ for all $i\geq 0$ has $\nu$-measure one.
    \item \label{prop:beclassical:2} Further, any point $x$ in this set is such that $\rho^{(n)}_x\rightarrow \delta_x$ in $\mathcal{P}(X)$.
\end{enumerate}
\end{prop}
\begin{proof}
For (\ref{prop:beclassical:1}), by classical L\'evy one has $\lim_n \mathbb{E}_{\nu}[I_{U_i} \mid \mathscr{F}_n]=I_{U_i}$ $\nu$-a.s. When written written out in terms of the disintegrations, this is $\lim_n \rho^{(n)}_x(U_i)=\delta_x(U_i)$ $\nu$-a.s.

We apply Portmanteau. Let $U$ be open, we show $\delta_x(U)\leq \liminf_n \rho^{(n)}_x(U)$. If $x$ is not in $U$, then this is trivial. Hence, suppose $x$ is in $U$. Since the sequence is a basis, choose open $U_i$ which is a subset of $U$ and which contains $x$. Then $\lim_n \rho^{(n)}_x(U_i)=1$ and so $\lim_n \rho^{(n)}_x(U)=1$.
\end{proof}

One effectivizes this by selecting the c.e. opens:


In philosophy, the most natural occurrence of lines is in two-dimensional semantics:
\begin{ex}\label{ex:2dsemantics} (Two dimensional semantics). Let $Y$ be a set of worlds, and let $Z$ be a set of perspectives, say of agents who take a stand or view about the worlds. Assume that $Y,Z$ are computable Polish spaces. Let $\lambda$ be a computable point of $\mathcal{P}(Y)$ and let $\mu$ be a computable point of $\mathcal{P}(Z)$. Intuitively, $\lambda$ can be thought of as an estimate for which world is more likely, and $\mu$ can be thought of as an estimate for which perspective is more likely. Then Borel subsets of $Y\times Z$ can be viewed as measurable propositions which have both a factual component and a subjective component. Let $\mathscr{F}$ be the $\sigma$-algebra on $Y\times Z$ consisting of sets of the form $U\times Z$ where $U$ ranges over c.e. opens from a $\lambda$-computable basis on $Y$. Then elements of the effective $\sigma$-algebra $\mathscr{F}$ are the measurable propositions where we have ``forgotten'' the subjective component and retained only the factual component. We might then think of $\mathscr{F}$ as the factual effective $\sigma$-algebra. The formula~(\ref{eqn:linesdisintegration}) can be interpreted as saying that given merely factual information, the conditional expectation of a two-dimensional random variable is obtained simply by fixing its factual component and averaging its perspectival component according to $\mu$.
\end{ex}

Here is the most simple version of ``lines'', the example from which it derives its name:
\begin{ex} (The simple version of lines). Let $a<b$ computable and let $X=[a,b]\times [a,b]$ and let $\nu$ be a computable point of $\mathcal{P}([0,1])$ such that that the open intervals $(p,q)$ for rational $a\leq p<q\leq b$ are a $\nu$-computable basis. Let $\mathscr{F}$ be the $\sigma$-algebra on $[a,b]\times [a,b]$ generated by sets of the form $(p,q)\times [a,b]$, where $a\leq p,q\leq b$ are rational. Then $\rho: [a,b]\times [a,b]\rightarrow \mathcal{P}([a,b]\times [a,b])$ given by $\rho_{(u,v)} = \delta_u \otimes \nu$ is a Martin-L\"of disintegration of $\mathscr{F}$, and one has the following expression for the version of conditional expectation, which for each $f$ in $\mathbb{L}_1(\nu\otimes \nu)$ is defined for $(\nu\otimes \nu)$-a.s. many $(u,v)$ in $X$:
\begin{equation*}
\mathbb{E}_{\nu\otimes \nu} [f \mid \mathscr{F}](u,v)=\int_a^b f(u,t) \; d\nu(t)
\end{equation*}
\end{ex}

Here are some very simple examples of partitions:
\begin{ex} (Effective partitions in Baire space given by length of string). Let $T\subseteq \mathbb{N}^{<\mathbb{N}}$ be any computable tree with no dead ends. Then $X=[T]$ is a computable Polish space. Let $\nu$ be a computable point of $\mathcal{P}(X)$. For $n\geq 1$, let $I_n=\{\sigma\in T: \left|\sigma\right|=n\}$ and let $\mathscr{F}_n$ be the effective partition $\{ [\sigma]: \sigma\in I_n\}$. Let $\rho^{(n)}:X\rightarrow \mathcal{M}^+(X)$ by $\rho^{(n)}_x=\sum_{\sigma\in I^+_n} \nu(\cdot \mid [\sigma])\cdot I_{[\sigma]}(x)$. Then $\rho$ is a Martin-L\"of disintegration of $\mathscr{F}_n$ and one has the following expression for the version of conditional expectation, which is defined for all $f$ in $\mathbb{L}_1(\nu)$ and all $x$ in $X$:
\begin{equation*}
\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x) = \sum_{\sigma\in I^+_n} \bigg(\frac{1}{\nu([\sigma])} \int_{[\sigma]} f \; d\nu\bigg) \cdot I_{\sigma}(x)
\end{equation*}
\end{ex}

\begin{ex} (Dyadic effective partitions of an interval with computable endpoints). Let $a<b$ be computable, so that the length $\ell=b-a$ of the interval $[a,b]$ is computable. Let $\nu$ be a computable point of $\mathcal{P}([a,b])$ which assigns probability zero to all computable reals. For $n\geq 1$, define the dyadic effective partition formed by cutting the interval $[a,b]$ into $2^n-1$ many half-open intervals of length $\frac{\ell}{2^n}$, and one closed interval of this same length: 
\begin{equation*}
\mathscr{D}_n=\{[a+i\cdot 2^{-n}\cdot \ell, a+(i+1)\cdot 2^{-n}\cdot \ell): 0\leq i<2^n-1]\}\cup \{[b-2^{-n}\cdot \ell, b]\}
\end{equation*}
Since $\nu$ assigns probability zero to all computable reals, the dyadic effective partition has the effective softening $\mathscr{D}_n^+ = \{A^{\circ}: A\in \mathscr{D}_n \; \& \; \nu(A)>0\}$ formed by removing the computable endpoints of the intervals. Let $\rho^{(n)}:X\rightarrow \mathcal{M}^+(X)$ by $\rho^{(n)}_x=\sum_{U\in \mathscr{D}_n^+} \nu(\cdot \mid U)\cdot I_{U}(x)$. Then $\rho^{(n)}$ is a Martin-L\"of disintegration of $\mathscr{D}_n$ with respect to $\nu$, and one has the following expression for the version of conditional expectation,which is defined for all $f$ in $\mathbb{L}_1(\nu)$ and all $x$ in $[a,b]$:
\begin{equation*}
\mathbb{E}_{\nu}[f\mid \mathscr{D}_n](x) = \sum_{U\in \mathscr{D}_n^+} \bigg(\frac{1}{\nu(U)} \int_U f \; d\nu\bigg) \cdot I_{U}(x)
\end{equation*}
\end{ex}


\begin{ex}\label{ex:dyadic} (Dyadic effective partitions of a $k$-dimensional unit cube with computable corners). Let $k\geq 1$ and let $\nu$ be a computable point of $\mathcal{P}([0,1]^k)$ which assigns probability zero to all cubes of dimension $<k$ which have computable corners. For $n\geq 1$, define the dyadic effective partition:
\begin{equation*}
\mathscr{D}_n^k = \{ \prod_{i=1}^k A_{k,i} : A_{k,i}\in \mathscr{D}_n\}
\end{equation*}
Since $\nu$  assigns probability zero to all cubes of dimension $<k$ which have computable corners, it has effective softening $\mathscr{D}_n^{k,+} = \{A^{\circ}: A\in  \mathscr{D}^k_n \; \& \; \nu(A)>0\}$ formed by removing the faces of the cube. Let $\rho^{(k,n)}:X\rightarrow \mathcal{M}^+(X)$ by $\rho^{(k,n)}_x=\sum_{U\in \mathscr{D}_n^{k,+}} \nu(\cdot \mid U)\cdot I_{U}(x)$. Then $\rho^{(k,n)}$ is a Martin-L\"of disintegrationn of $\mathscr{D}_n^k$ with respect to $\nu$, and one has the following expression for the version of conditional expectation, which is defined for all $f$ in $\mathbb{L}_1(\nu)$ and all $(x_1, \ldots, x_k)$ in $[a,b]^k$:
\begin{equation*}
\mathbb{E}_{\nu}[f\mid \mathscr{D}_n^k](x_1, \ldots, x_k) = \sum_{U\in \mathscr{D}_n^{k,+}} \bigg(\frac{1}{\nu(U)} \int_U f \; d\nu\bigg) \cdot I_{U}(x_1, \ldots, x_k)
\end{equation*}
\end{ex}

The following proposition is a technical proposition which we need to handle the $p=1$ case of Theorem~\ref{thm:newnewlevy}:
\begin{prop}\label{prop:mlrgotozeroL0}
Suppose that $\nu$ is a computable point of $\mathcal{P}(X)$.
\begin{enumerate}[leftmargin=*]
    \item \label{prop:mlrgotozeroL0:1} If $x$ in $\mathsf{MLR}^{\nu}$, then $x$ is in $\mathsf{KR}^{\nu}$ and  $f_s(x)\rightarrow 0$ for all uniformly lsc $f_s:X\rightarrow [0,\infty]$ with $f_s\rightarrow 0$ in $L_0(\nu)$ at a geometric rate of convergence.
    \item \label{prop:mlrgotozeroL0:2} Suppose $x$ in $\mathsf{KR}^{\nu}$. Suppose for all uniformly lsc $f_s:X\rightarrow [0,\infty]$ with $f_s\rightarrow 0$ in $L_0(\nu)$ at a geometric rate of convergence, one has $f_s(x)\rightarrow 0$. Then $f(x)<\infty$ for every lsc $f:X\rightarrow [0,\infty]$ which is a computable point of $L_0(\nu)$.
    \item \label{prop:mlrgotozeroL0:3} If there is a $\nu$-computable basis consisting of clopens, then the hypothesis of ``$x$ being in $\mathsf{KR}^{\nu}$'' can be removed from the previous~item.
\end{enumerate}
\end{prop}

\begin{proof}
For (\ref{prop:mlrgotozeroL0:1}), suppose that rational $b>1$ is the rate of convergence. Let $U_s$ be the c.e. open $\{x\in X: f_s(x)>b^{-s}\}$, so that $\nu(U_s)<b^{-s}$. Then $f=\sum_s I_{U_s}$ is non-negative lsc. And $f$ is in $L_1(\nu)$ since $\mathbb{E}_{\nu} f = \sum_s \nu(U_s) \leq \sum_s b^{-s} <\infty$. Let $x$ in $\mathsf{MLR}^{\nu}$. Since $x$ is in $\mathsf{MLR}^{\nu}$, we have $f(x)<\infty$ and hence there is $s_0\geq 0$ such that for all $s\geq s_0$ one has that $x$ not in $U_{s}$. Hence $f_s(x)\leq b^{-s}$ for all $s\geq s_0$. This implies that $f_s(x)\rightarrow 0$.

For (\ref{prop:mlrgotozeroL0:2}), suppose that $f:X\rightarrow [0,\infty]$ is lsc and $L_0(\nu)$ computable. By Propositions~\ref{prop:exptoflsc}, \ref{prop:lscL0}, choose a computable sequence $f_s$ from the countable dense set of $L_0(\nu)$ such that $f_s\leq f_{s+1}$ everywhere and $f=\sup_s f_s$ everywhere and $f_s\rightarrow f$ fast in $L_0(\nu)$. By Proposition~\ref{prop:shiftbasistolpst}, let $\breve{f}_s$ be non-negative usc equal to $f_s$ on $\mathsf{KR}^{\nu}$. Hence $-\breve{f}_s$ is lsc and $f-\breve{f}_s$ is lsc. Let $h_s=\max(0, f-\breve{f}_s)$, which is non-negative lsc. Further, we have that $h_s\rightarrow 0$ fast in $L_0(\nu)$. Hence by hypothesis, $h_s(x)\rightarrow 0$. Since $x$ is in $\mathsf{KR}^{\nu}$, we then have that $f_s(x)\rightarrow f(x)$, which implies that $f(x)<\infty$.

For (\ref{prop:mlrgotozeroL0:3}), suppose that there is a $\nu$-computable basis consisting of clopens and $x$ is such that $f_s(x)\rightarrow 0$ for all uniformly lsc $f_s:X\rightarrow [0,\infty]$ with $f_s\rightarrow 0$ in $L_0(\nu)$ at a geometric rate of convergence. We show that $x$ is in $\mathsf{KR}^{\nu}$. Suppose that $U$ is c.e. open with $\nu(U)=1$. Let $U=\bigcup_n C_n$, where $C_n$ is a computable sequence from the $\nu$-computable basis of clopens, where without loss of generality we may assume that $C_n\subseteq C_{n+1}$. Let $V_n=X\setminus C_n$, which is also clopen, and so that we have $V_n\supseteq V_{n+1}$. Then $I_{V_n}$ is an $L_1(\nu)$ Schnorr test with $I_{V_n}\rightarrow 0$ in $L_1(\nu)$. Since $L_1(\nu)$ computably embeds in $L_0(\nu)$, we have that $I_{V_n}\rightarrow 0$ in $L_0(\nu)$. Since this is a computable sequence in $L_0(\nu)$, we can compute a subsequence such that  $I_{V_n}\rightarrow 0$ fast in $L_0(\nu)$. Then by hypothesis $I_{V_n}(x)\rightarrow 0$. This implies that $x$ is eventually not in $V_n$ and so eventually in $C_n$ and hence in~$U$.
\end{proof}



% Sometimes it is useful to state the abstract version of lines where the $\sigma$-algebra inverts the roles of the two coordinates:
% \begin{prop}\label{prop:linesdisintegration:permute}  (The abstract version of lines, with reverse order). 
% Suppose that $Y,Z$ are computable Polish spaces. Suppose that $\lambda$ is a computable point of $\mathcal{P}(Y)$ and $\mu$ is a computable point of $\mathcal{P}(Z)$. Let $\mathscr{F}$ be the $\sigma$-algebra on $Y\times Z$ generated by sets of the form $Y\times V$, where $V$ ranges over c.e. opens from a $\mu$-computable basis on $Z$. Then $\rho: Y\times Z\rightarrow \mathcal{P}(Y\times Z)$ given by $\rho_{(u,v)} = \lambda\otimes\delta_v$ is a Martin-L\"of disintegration of $\mathscr{F}$ with respect to $\lambda \otimes \mu$, and one has the following expression for the version of conditional expectation, which for each $f$ in $\mathbb{L}_1(\lambda\otimes\mu)$ is defined for $(\lambda \otimes \mu)$-a.s. many $(u,v)$ in $Y\times Z$:
% \begin{equation}\label{eqn:linesdisintegrationv5}
% \mathbb{E}_{\lambda\otimes\mu} [f \mid \mathscr{F}](u,v)=\int_Y f(s,v) \; d\lambda(s)
% \end{equation}
% \end{prop}


Finally, we can combine partitions and lines as follows:
\begin{prop}\label{prop:combinepartitionslines1}
(Abstract version of a combination of partitions and lines). 

Suppose that $Y,Z$ are computable Polish spaces. Suppose that $\lambda$ is a computable point of $\mathcal{P}(Y)$ and $\mu$ is a computable point of $\mathcal{P}(Z)$. 

Consider the effective partition $\{C_i: i\in I\}$ of $Z$ with effective softening $\{V_i: i\in I\}$.

Let $\mathscr{F}$ be the $\sigma$-algebra on $Y\times Z$ generated by sets of the form $U\times C_i$, where $U$ ranges over c.e. opens from a $\lambda$-computable basis on $Y$. Then the map $\rho: Y\times Z\rightarrow \mathcal{M}^+(Y\times Z)$ given by $\rho_{(u,v)} = \sum_{i\in I^+} \big(\delta_u\otimes \mu(\cdot \mid V_i)\big)\cdot I_{V_i}(v)$ is a Martin-L\"of disintegration of $\mathscr{F}$ with respect to $\lambda \otimes \mu$, and one has the following expression for the version of conditional expectation:
\begin{equation}\label{eqn:combinepartitionslines1}
\mathbb{E}_{\lambda\otimes\mu} [f \mid \mathscr{F}](u,v)= \sum_{i\in I^+} \bigg(\frac{1}{\mu(V_i)} \int_{V_i} f(u,t) \; d\mu(t)\bigg) \cdot I_{V_i}(v)
\end{equation}
\end{prop}
\begin{proof}
This proof is just a simple combination of the proofs of Proposition~\ref{prop:partitionsaredisintegrations} and Proposition~\ref{prop:linesdisintegration}. 

%% most likely comment this proof out after this point.

As in the proof of Proposition~\ref{prop:partitionsaredisintegrations}, by the definition of effective softening, the sets $V_i, V_j$ for distinct $i,j$ in $I^+$ have empty intersection. Hence, the map $\rho$ has codomain $\mathcal{M}^+(Y\times Z)$. In particular, if $v$ in $V_i$ for $i$ in $I^+$, then $\rho_{(u,v)}=\delta_u\otimes \mu(\cdot \mid V_i)$, which is in $\mathcal{P}(Y\times Z)$ and hence in $\mathcal{M}^+(Y\times Z)$. But if $v$ not in any $V_i$ for $i$ in $I^+$, then $\rho_{(u,v)}=0$, which is a point of $\mathcal{M}^+(Y\times Z)$.


Note that $\frac{d\nu(\cdot \mid V_i)}{d\mu}=\frac{1}{\mu(V_i)}\cdot I_{V_i}$ for $i$ in $I^+$. Second that one has the following for $f$ in $\mathbb{L}_1(\lambda\otimes \mu)$, by Fubini-Tonelli, and by the same theorem is defined for $\lambda$-a.s. many $u$ in $Y$, and hence for $(\lambda \otimes \mu)$-a.s. many $(u,v)$ in $Y\times Z$:
\begin{align*}
& \mathbb{E}_{\lambda\otimes\mu} [f \mid \mathscr{F}](u,v)= \sum_{i\in I^+} \bigg( \int_Z \int_Y f(s,t) \; d\delta_u(s) \;  d\mu(\cdot \mid V_i)(t) \bigg) \cdot I_{V_i}(v)   \\
= & \sum_{i\in I^+}  \bigg( \int_Z f(u,t) \; d\mu(\cdot \mid V_i)(t) \bigg) \cdot I_{V_i}(v) = \sum_{i\in I^+}  \bigg( \frac{1}{\mu(V_i)} \int_{V_i} f(u,t) \; d\mu(t) \bigg) \cdot I_{V_i}(v) 
\end{align*}
When we integrate over $v$ in $C_j$ for $j$ in $I^+$, we then get:
\begin{equation*}
\int_{C_j} \mathbb{E}_{\lambda\otimes\mu} [f \mid \mathscr{F}](u,v) \; d\mu(v)  = \int_{V_j} f(u,t) \; d\mu(t)
\end{equation*}
Hence if $j$ in $I^+$ and $B\subseteq Y$ is Borel we have by Fubini-Tonelli that:
\begin{equation*}
 \int_{B\times C_j}  \mathbb{E}_{\lambda\otimes\mu} [f \mid \mathscr{F}](u,v) \; d(\lambda \otimes \mu)(u,v) = \int_B  \int_{V_j} f(u,t) \; d\mu(t) \; d\lambda(u) = \int_{B\times C_j} f(u,t) \; d(\lambda \otimes \mu)(u,t)
\end{equation*}
By contrast, if $j$ is not in $I^+$, then $C_j$ is $\mu$-null and hence $B\times C_j$ is $(\lambda\otimes \mu)$-null for any Borel $B\subseteq Y$, and we trivially have 
\begin{equation*}
 \int_{B\times C_j}  \mathbb{E}_{\lambda\otimes\mu} [f \mid \mathscr{F}](u,v) \; d(\lambda \otimes \mu)(u,v) = \int_{B\times C_j} f(u,t) \; d(\lambda \otimes \mu)(u,t)
\end{equation*}
This shows that (\ref{eqn:combinepartitionslines1}) is a version of the conditional expectation of $\mathscr{F}$ with respect to $\lambda\otimes \mu$.

Note that $[(u,v)]_{\mathscr{F}}= \{u\}\times C_j$ where $v$ is in $C_j$. Recall that $\mathsf{KR}^{\lambda\otimes \mu}(Y\times Z)=\mathsf{KR}^{\lambda}(Y)\times \mathsf{KR}^{\mu}(Z)$. Suppose that $(u,v)$ in $\mathsf{KR}^{\lambda\otimes \mu}(Y\times Z)$.  Then one has
\begin{equation*}
[(u,v)]_{\mathscr{F}} \cap \mathsf{KR}^{\lambda\otimes \mu}(Y\times Z) = (\{u\}\cap \mathsf{KR}^{\lambda}(Y))\times (C_j\cap  \mathsf{KR}^{\mu}(Z)) = \{u\}\times (V_j\cap \mathsf{KR}^{\mu}(Z))
\end{equation*}
From this we get $\rho_{(u,v)}([(u,v)]_{\mathscr{F}}\cap \mathsf{KR}^{\lambda\otimes \mu}(Y\times Z)) = \delta_u(\{u\}) \cdot \mu(V_j\cap \mathsf{KR}^{\mu}(Z)\mid V_j)=1$.

For Schnorr disintegrations, suppose that $(u,v)$ is in $\mathsf{SR}^{\lambda \otimes \mu}(Y\times Z)$, so that $u$ is in $\mathsf{SR}^{\lambda}(Y)$. Since $[(u,v)]_{\mathscr{F}}= \{u\}\times C_j$ where $v$ is in $C_j$, we want to show that $(\delta_u\otimes \mu(\cdot\mid V_j))(A)=1$, where $A$ is the event $(\{u\}\times C_j)\cap \mathsf{SR}^{\lambda \otimes \mu}(Y\times Z)$. For $s$ in $Y$, we have $A_s=\{t\in C_j: s=u \wedge (s,t)\in \mathsf{SR}^{\lambda \otimes \mu}(Y\times Z)\}$. By choosing ${\bf a}$ which computes a fast Cauchy sequence for $u$, we have by van Lambalgen's Theorem that $A_u\supseteq C_j\cap \mathsf{SR}^{\mu, {\bf a}}(Z)$ and so $\mu(A_u\mid C_j)=1$. Hence it follows by Fubini-Tonelli that $\rho_{(u,v)}(A)=(\delta_u\otimes \mu(\cdot \mid V_j))(A)=\int_Y \mu(A_s\mid V_j)\; d\delta_u(s) = \mu(A_u\mid V_j) =1$, which is what we wanted to show. The argument for Martin-L\"of disintegrations is similar.

Suppose that $\mathcal{O}\subseteq Y\times Z$ is c.e. open. Then we can write $V=\bigcup_i U_i\times W_i$ where $U_i\subseteq Y, W_i\subseteq Z$ are computable sequences of c.e. opens with $U_i\subseteq U_{i+1}$ and $W_i\subseteq W_{i+1}$. Then for rational $q\geq 0$, we have $\rho_{u,v}(\mathcal{O})>q$ iff there is $i\geq 0$ with $\rho_{(u,v)}(U_i\times W_i)>q$, which happens iff there is $i\geq 0$ and $j\in I^+$ with $\delta_u(U_i)\cdot \mu(W_i\mid V_j)\cdot I_{V_j}(v)>q$, which happens iff there is $i\geq 0$ and $j$ in $I^+$ with $u$ in $U_i$ and $v$ in $V_j$ and $\mu(W_i\mid V_j)>q$. This is obviously a c.e. open condition in variables $(u,v)$.
\end{proof}


==> zzz-temp.tex <==
% southeast
\draw[semithick] (1+0, 0) -- (1+.475, 0);
\draw[semithick] (1+.525, 0) -- (1+.975, 0);
\draw[semithick] (1+0, .525) -- (1+.475, .525);
\draw[semithick] (1+0, .525) -- (1+0, .975);
\draw[semithick, dotted] (1+0, .975) -- (1+.475, .975);
\draw[semithick, dotted] (1+.475, 1) -- (1+.475, .525);
\draw[semithick, dotted] (1+.475, .475) -- (1+.475, 0);
\draw[semithick] (1+0, 0) -- (1+0, .475);
\draw[semithick, dotted] (1+0, .475) -- (1+.475, .475);
\draw[semithick, dotted] (1+.525, .475) -- (1+1, .475);
\draw[semithick, dotted] (1+0, 0) -- (1+0, .475);
\draw[semithick, dotted] (1+0, .475) -- (1+.475, .475);
\draw[semithick] (1+.525, 0) -- (1+.525, .475);
\draw[semithick, dotted] (1+1, 0) -- (1+1, .475);
\draw[semithick] (1+.525, .525) -- (1+.525, .975);
\draw[semithick] (1+.525, .525) -- (1+.975, .525);
\draw[semithick, dotted] (1+.975, .525) -- (1+.975, .975);
\draw[semithick, dotted] (1+.975, .975) -- (1+.525, .975);
% northeast
\draw[semithick] (1+0, 0+1) -- (1+.475, 0+1);
\draw[semithick] (1+.525, 0+1) -- (1+.975, 0+1);
\draw[semithick] (1+0, .525+1) -- (1+.475, .525+1);
\draw[semithick] (1+0, .525+1) -- (1+0, .975+1);
\draw[semithick, dotted] (1+0, .975+1) -- (1+.475, .975+1);
\draw[semithick, dotted] (1+.475, 1+1) -- (1+.475, .525+1);
\draw[semithick, dotted] (1+.475, .475+1) -- (1+.475, 0+1);
\draw[semithick] (1+0, 0+1) -- (1+0, .475+1);
\draw[semithick, dotted] (1+0, .475+1) -- (1+.475, .475+1);
\draw[semithick, dotted] (1+.525, .475+1) -- (1+1, .475+1);
\draw[semithick, dotted] (1+0, 0+1) -- (1+0, .475+1);
\draw[semithick, dotted] (1+0, .475+1) -- (1+.475, .475+1);
\draw[semithick] (1+.525, 0+1) -- (1+.525, .475+1);
\draw[semithick, dotted] (1+1, 0+1) -- (1+1, .475+1);
\draw[semithick] (1+.525, .525+1) -- (1+.525, .975+1);
\draw[semithick] (1+.525, .525+1) -- (1+.975, .525+1);
\draw[semithick, dotted] (1+.975, .525+1) -- (1+.975, .975+1);
\draw[semithick, dotted] (1+.975, .975+1) -- (1+.525, .975+1);
% northwest
\draw[semithick] (0, 0+1) -- (.475, 0+1);
\draw[semithick] (.525, 0+1) -- (.975, 0+1);
\draw[semithick] (0, .525+1) -- (.475, .525+1);
\draw[semithick] (0, .525+1) -- (0, .975+1);
\draw[semithick, dotted] (0, .975+1) -- (.475, .975+1);
\draw[semithick, dotted] (.475, 1+1) -- (.475, .525+1);
\draw[semithick, dotted] (.475, .475+1) -- (.475, 0+1);
\draw[semithick] (0, 0+1) -- (0, .475+1);
\draw[semithick, dotted] (0, .475+1) -- (.475, .475+1);
\draw[semithick, dotted] (.525, .475+1) -- (1, .475+1);
\draw[semithick, dotted] (0, 0+1) -- (0, .475+1);
\draw[semithick, dotted] (0, .475+1) -- (.475, .475+1);
\draw[semithick] (.525, 0+1) -- (.525, .475+1);
\draw[semithick, dotted] (1, 0+1) -- (1, .475+1);
\draw[semithick] (.525, .525+1) -- (.525, .975+1);
\draw[semithick] (.525, .525+1) -- (.975, .525+1);
\draw[semithick, dotted] (.975, .525+1) -- (.975, .975+1);
\draw[semithick, dotted] (.975, .975+1) -- (.525, .975+1);


Again, to illustrate:
\begin{ex}\label{ex:product:martingales:2}
Suppose that $f_n:X\rightarrow [0,\infty]$ is a sequence of independent $L_2(\nu)$ Schnorr tests with $\mathbb{E}_{\nu} f_n=1$ for all $n\geq 1$. Suppose that $\mathscr{F}_n=\sigma(f_1, \ldots, f_n)$ is an effective filtration equipped with Schnorr disintegrations which is almost~full. Let  $M_n=\prod_{i=1}^n f_i$. Then $\lim_n M_n$ exists on $\mathsf{SR}^{\nu}$.

For instance, if $X=2^{\mathbb{N}}$ and $\nu$ is the fair coin toss measure, then for any $\omega$ in  $\mathsf{SR}^{\nu}$, one has that the following infinite product exists:
\begin{equation*}
\prod_n (\omega(n)+\frac{1}{2})
\end{equation*}
One can see this by using the Schnorr disintegrations from Proposition~\ref{prop:partitionsaredisintegrations} and by appealing to fullness from Proposition~\ref{prop:effectshrinking} and by using $f_n(\omega)=\omega(n)+\frac{1}{2}$. Indeed, one has $\mathbb{E}_{\nu} f_n = 1$ and $\|f_n\|_2 =\frac{\sqrt{5}}{2}$ and so $\|M_n\|_2=(\frac{\sqrt{5}}{2})^n$
\end{ex}



\begin{prop}
Let $\nu$ be a computable point of $\mathcal{P}(2^{\mathbb{N}})$ with full support. 

There is Turing program $e$ such that:
\begin{itemize}[leftmargin=*]
\item $W_e^{\omega}$ is infinite for all $\omega$ in $2^{\mathbb{N}}$.
\item $V_m=\{\omega: m\in W_e^{\omega}\}$ has uniformly computable $\nu$-measure.
\item There is $\omega$ in $\mathsf{SR}^{\nu}$ such that $W_e^{\omega}$ is not Turing computable in $\omega$.
\end{itemize}
\end{prop}
\begin{proof}
Since $\nu$ has full support, let $U_n$ be a sequential Schnorr $\nu$-test such that each $U_n$ is dense. Then define:
\begin{equation*}
W_e^{\omega} = \{2m: \omega\in U_m\}\cup \{2m+1: m\geq 0\}
\end{equation*}
Then $V_{2m} = U_m$ and $V_{2m+1}=2^{\mathbb{N}}$. Then we claim that there is $\omega$ in $\mathsf{SR}^{\nu}$ such that $W_e^{\omega}$ is not Turing computable in $\omega$. Suppose not. Then every $\omega$ in $\mathsf{SR}^{\nu}$ is such that $W_e^{\omega}$ is Turing computable in $\omega$. Then there is Turing program $i$ such that $\nu(S_i)>0$, where 
\begin{equation*}
S_i = \{\omega\in \mathsf{SR}^{\nu} : W_i^{\omega}=\mathbb{N}\setminus W_e^{\omega}\}
\end{equation*}
By Lebesgue density, choose a point $\omega^{\prime}$ in $S_i$ and an $n_0\geq 0$ such that $\nu(S_i \mid [\omega^{\prime}\upharpoonright n])>\frac{1}{2}$ for all $n\geq n_0$.

\end{proof}

\begin{prop}
Let $\nu$ be a computable point of $\mathcal{P}(2^{\mathbb{N}})$ with full support. 

There is Turing program $e$ such that:
\begin{itemize}[leftmargin=*]
\item $W_e^{\omega}$ is infinite for all $\omega$ in $2^{\mathbb{N}}$.
\item $V_m=\{\omega: m\in W_e^{\omega}\}$ has uniformly computable $\nu$-measure.
\item There is $\omega$ in $\mathsf{SR}^{\nu}$ such that $W_e^{\omega}$ is not Turing computable in $\omega$.
\end{itemize}
\end{prop}
\begin{proof}
Since $\nu$ has full support, let $U_n$ be a sequential Schnorr $\nu$-test such that each $U_n$ is dense. Then define:
\begin{equation*}
W_e^{\omega} = \{2m: \omega\in U_m\}\cup \{2m+1: m\geq 0\}
\end{equation*}
Then $V_{2m} = U_m$ and $V_{2m+1}=2^{\mathbb{N}}$. Then we claim that there is $\omega$ in $\mathsf{SR}^{\nu}$ such that $W_e^{\omega}$ is not Turing computable in $\omega$. Suppose not. Then every $\omega$ in $\mathsf{SR}^{\nu}$ is such that $W_e^{\omega}$ is Turing computable in $\omega$. Then for every $\omega$ in $\mathsf{SR}^{\nu}$ there is Turing procedure $i$ such that $W_i^{\omega}=\mathbb{N}\setminus W_e^{\omega}$. Since for every $\omega$ in $\mathsf{SR}^{\nu}$ there is $m$ with $\omega\notin U_m$, we have that for every $\omega$ in $\mathsf{SR}^{\nu}$ there is $i,m\geq 0$ such that $W_i^{\omega}=\mathbb{N}\setminus W_e^{\omega}$ and $2m\in W_i^{\omega}$. Then there is $i,m\geq 0$ such that $\nu(S_{i,m})>0$, where we define
\begin{equation*}
S_{i,m} = \{\omega\in \mathsf{SR}^{\nu} : W_i^{\omega}=\mathbb{N}\setminus W_e^{\omega} \; \& \;  2m\in W_i^{\omega}\}
\end{equation*}
By the Lebesgue Density Theorem, choose $\omega_0$ in this set such that $\lim_s \nu(S_{i,m}\mid [\omega_0\upharpoonright s])=1$. Choose $s_0\geq 0$ such that $2m$ in $W_{i,s_0}^{\omega}$. Choose $s_1\geq s_0$ such that $\nu(S_{i,m}\mid [\omega_0\upharpoonright s])>\frac{3}{4}$ for all $s\geq s_1$. Let $s\geq s_1$. Then $\frac{3}{4}<\nu(S_{i,m}\mid [\omega_0\upharpoonright s])\leq \nu(X\setminus U_m\mid  [\omega_0\upharpoonright s])$.
\end{proof}

SW working \today:
\begin{prop}
Let $\nu$ be uniform measure on Cantor space. There is a computable sequence of c.e. opens $V_{n,m}$ such that 
\begin{itemize}
\item $V_{n,m}$ has uniformly computable $\nu$-measure.
\item Each $\omega$ in Cantor space is in infinitely many of the $V_{n,m}$.
\item There is $\omega$ in $\mathsf{SR}^{\nu}$ such that $W_e^{\omega}\nleq_T \omega$, where $W_e^{\omega}:=\{(n,m): \omega\in V_{n,m}\}$
\end{itemize}
\end{prop}
\begin{proof}
Recall that an element $\omega$ of Cantor space is called \emph{left-c.e.} if the set $L(\omega):=\{\sigma: \sigma<_{lex} \omega\}$ is a c.e. set.\footnote{\cite[51]{Nies2008aa}.} There is a universal enumeration $\omega_0, \omega_1, \ldots$ of the left-c.e. elements of Cantor space, given by taking the universal enumeration of c.e. subsets of $2^{<\mathbb{N}}$ and closing downward. Choose some fixed computable sequence $\sigma_{n,m}$ such that for each $n\geq 0$ one has that $\sigma_{n,0},\sigma_{n,1},\ldots$ enumerates $L_{\omega_n}$. Let $V_{n,m}=[\sigma_{n,m}]$, and let $V_{\infty,m}=[1^m]$. 

Then by construction $V_{n,m}$ has uniformly computable $\nu$-measure. 

Further, each $\omega\neq \overline{1}$ in Cantor space is in infinitely many of the $V_{n,m}$ since the left-c.e. elements are dense in $2^{\mathbb{N}}\setminus \{\overline{1}\}$, and obviously $\overline{1}$ is in each $V_{\infty,m}$. 

For reductio, suppose that each $\omega$ in $\mathsf{SR}^{\nu}$ is such that such that $W_e^{\omega}\nleq_T \omega$.

There is a pair of high c.e. degrees which are a minimal pair.\footnote{\cite{Miller1981-bd}, \cite[827]{Shore1993-ss}.} Each high c.e. degree contains a left-c.e. computably random set.\footnote{\cite[280]{Nies2008aa}.}, and hence a left-c.e. Schnorr random set. 

Hence, choose two left c.e. Schnorr randoms $\omega_0, \omega_1$ which form a minimal pair. Without loss of generality $\omega_0<_{lex} \omega_1$.


\end{proof}




*****

\section{Rates of convergence to the truth}

\begin{defn}
Suppose that $X$ is a computable Polish space and $\nu$ is a computable probability measure. Suppose that $\mathscr{F}_n$ is an almost-full effective filtration, equipped with Kurtz disintegrations. Let $p\geq 1$ be computable. 

One says that \emph{$\mathsf{SR}^{\nu}$ has computable rates of convergence to the truth for individual $L_p(\nu)$ Schnorr tests} if for every $L_p(\nu)$ Schnorr test and every $x$ in $\mathsf{SR}^{\nu}$ with $x_k\rightarrow x$ fast there is an $\{x_k:k\geq 0\}$-computable function $r: \mathbb{Q}^{>0}\rightarrow \mathbb{N}$ such that for all rational $\epsilon>0$ and $n\geq r(m,\epsilon)$ one has $\left|\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)-f(x)\right|<\epsilon$.

One says that \emph{$\mathsf{SR}^{\nu}$ has computable rates of convergence to the truth for families of $L_p(\nu)$ Schnorr tests} if for every computable sequence $f_m$ of $L_p(\nu)$ Schnorr tests and every $x$ in $\mathsf{SR}^{\nu}$ with $x_k\rightarrow x$ fast there is an $\{x_k:k\geq 0\}$-computable function $r:\mathbb{N}\times \mathbb{Q}^{>0}\rightarrow \mathbb{N}$ such that for all $m\geq 0$ and rational $\epsilon>0$ and $n\geq r(m,\epsilon)$ one has $\left|\mathbb{E}_{\nu}[f_m\mid \mathscr{F}_n](x)-f(x)\right|<\epsilon$.
\end{defn}


\begin{prop}
Let $X$ be Cantor space and let $\nu$ be uniform measure on Cantor space and let $\mathscr{F}_n$ be the filtration of length $n$ strings equipped with the Martin-L\"of disintegration $\rho^{(n)}_{\omega} = \sum_{\left|\sigma\right|=n} \nu(\cdot \mid [\sigma])\cdot I_{[\sigma]}$.

Then $\mathsf{SR}^{\nu}$ does not have computable rates of convergence to the truth for families of $L_p(\nu)$ Schnorr tests.
\end{prop}
\begin{proof}
Define the computable sequence of c.e. opens $U_{\sigma,e}=\bigcup_s U_{\sigma,e,s}$, where 
\begin{equation*}
U_{\sigma, e, s} = \begin{cases}
\bigcup_{t=0}^s [\sigma\, 0^t\, 1]      & \text{if $\varphi_{e,s}(e)\upparrow$,} \\
\bigcup_{t=0}^{s_0} [\sigma\, 0^t\, 1]      & \text{if $\varphi_{e,s_0}(e)\ddownarrow$ for least $s_0\leq s$}.
\end{cases}
\end{equation*}
The $\nu$-measure of these c.e. opens is as follows:
\begin{equation*}
\nu(U_{\sigma, e}) = \begin{cases}
2^{-\left|\sigma\right|}      & \text{if $\varphi_{e}(e)\upparrow$,} \\
2^{-\left|\sigma\right|} \cdot \sum_{t=0}^{s_0}  2^{-(t+1)}
    & \text{if $\varphi_{e}(e)\ddownarrow$ for least $s_0s$}.
\end{cases}
\end{equation*}
These are computable reals since the computable sequence $q_{\sigma,e,s}\rightarrow \nu(U_{\sigma,e})$ fast, where
\begin{equation*}
q_{\sigma, e, s} = \begin{cases}
2^{-\left|\sigma\right|+1} \cdot \sum_{t=0}^{s}  2^{-(t+1)}     & \text{if $\varphi_{e,s}(e)\upparrow$,} \\
2^{\left|\sigma\right|+} \cdot \sum_{t=0}^{s_0}  2^{-(t+1)}      & \text{if $\varphi_{e,s_0}(e)\ddownarrow$ for least $s_0\leq s$}.
\end{cases}
\end{equation*}

Let $f_{\sigma,e}=I_{U_{\sigma,e}}$, which is a computable sequence of $L_1(\nu)$ Schnorr tests. 

Suppose that $\omega$ is an $\mathsf{SR}^{\nu}$ such that $\omega<_T \emptyset^{\prime}$. 

Suppose for reductio that there is an $\omega$-computable function $r:2^{<\mathbb{N}}\times \mathbb{N}\times \mathbb{Q}^{>0}\rightarrow \mathbb{N}$ such that for all $\sigma$ in $2^{<\mathbb{N}}$ and $e\geq 0$ and rational $\epsilon>0$ and $n\geq r(\sigma,e,\epsilon)$ one has $\left|\nu(U_{\sigma,e}\mid [\omega\upharpoonright n])-I_{U_{\sigma,e}}(\omega)\right|<\epsilon$.

Using this assumption, we now argue that $\omega$ does compute $\emptyset^{\prime}$. Suppose that $e\geq 0$ is given. Then for all $\ell\geq 0$ and $n\geq r(\omega\upharpoonright \ell, e, 2^{-\ell})$ and $n\geq \ell$ one has that $\left|\nu(U_{\omega\upharpoonright \ell,e}\mid [\omega\upharpoonright n])-I_{U_{\omega\upharpoonright \ell,e}}(\omega)\right|<2^{-\ell}$.

\end{proof}



\begin{prop}
Let $\nu$ be Lebesgue measure on Cantor space. 

Then there is a computable sequence of c.e. opens $V_i$ such that
\begin{enumerate}[leftmargin=*]
\item \label{check:1} $V_i$ has uniformly computable $\nu$-measure.
\item \label{check:2} Each $\omega$ in Cantor space is in infinitely many of the $V_i$.
\item \label{check:3} There is $\omega$ in $\mathsf{SR}^{\nu}$ such that $W_e^{\omega}\nleq_T \omega$, where $W_e^{\omega}:=\{i: \omega\in V_i\}$
\end{enumerate}
\end{prop}
\begin{proof}
Define $V_{2i}$ to be the c.e. open $\bigcup_s V_{2i,s}$, where we define:
\begin{equation*}
V_{2i,s} = \begin{cases}
\bigsqcup_{t\leq s} [1^t \, 0]      & \text{if $\varphi_{i,s}(i)\upparrow$}, \\
\bigsqcup_{t\leq s_0} [1^t \, 0]      & \text{if $\varphi_{i,s_0}(i)\ddownarrow$ for some least $s_0\leq s$}.
\end{cases}
\end{equation*}
Then note that $V_{2i}$ has the following $\nu$-measure:
\begin{equation*}
\nu(V_{2i}) = \begin{cases}
1      & \text{if $\varphi_{i}(i)\upparrow$}, \\
\sum_{t\leq s_0} 2^{-(t+1)}      & \text{if $\varphi_{i,s_0}(i)\ddownarrow$ for some least $s_0$}.
\end{cases}
\end{equation*}
Note that $V_{2i}$ has computable $\nu$-measure $q_{2i,s}\rightarrow \nu(V_{2i})$ fast, where 
\begin{equation*}
q_{2i,s} = \begin{cases}
\sum_{t\leq s} 2^{-(t+1)}       & \text{if $\varphi_{i,s}(i)\upparrow$}, \\
\sum_{t\leq s_0} 2^{-(t+1)}       & \text{if $\varphi_{i,s_0}(i)\ddownarrow$ for some least $s_0\leq s$}.
\end{cases}
\end{equation*}
Finally, let $V_{2i+1}=[1^i]$, so that it is also a c.e. open when uniformly computable $\nu$-measure. On the basis of this construction, we then have (\ref{check:1}). And (\ref{check:2}) follows from the halting set $\emptyset^{\prime}$ being coinfinite.

For (\ref{check:3}), let $\omega$ in $\mathsf{SR}^{\nu}$. Let $n$ be least such that $\omega$ is in $[1^n 0]$. Then
\begin{equation*}
\{ j: \omega\in V_j\} = \{2i: \varphi_i(i)\upparrow\} \cup \{ 2i: \exists \;  s_0\geq n \; \varphi_{i,s_0}(i)\ddownarrow \; \& \; \forall\; s<s_0 \; \varphi_{i,s_0}(i)\upparrow\}
\end{equation*}

\end{proof}




\begin{thm}\label{thm:rates2}
Let $X$ be Cantor space, and let $\nu$ be uniform measure. Let $\mathscr{F}_n$ be the full filtration generated by the length $n$ strings, equipped with the effective Martin-L\"of disintegration $\rho^{(n)}=\sum_{\left|\sigma\right|=n} \nu(\cdot \mid [\sigma])\cdot I_{[\sigma]}$, which results in the version $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](\omega) = \frac{1}{\nu([\omega\upharpoonright n])} \int_{[\omega\upharpoonright n]} f \; d\nu$.

Then it is \emph{not} the case that: for every $L_1(\nu)$ Schnorr test $f$ and every  $x$ in $\mathsf{SR}^{\nu}$ there is a computable function $m:\mathbb{Q}^{>0}\rightarrow \mathbb{N}$ such that for all rational $\epsilon>0$ and all $n\geq m(\epsilon)$ one has $\left|\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)-f(x)\right|<\epsilon$.
\end{thm}
\begin{proof}
In this proof, we use $\mathrm{cl}_X(U)$ for the topological closure of set $U$ in space $X$. 

Let $U$ be a c.e. open with $0<\nu(U)<1$ computable and $\nu(\mathrm{cl}_X(U))=1$  (cf. discussion after Definition~\ref{defn:eff:cantor}). Let $f=I_U$, which is an $L_1(\nu)$ Schnorr test.

Suppose for reductio that $\mathsf{SR}^{\nu}(X)$ is a subset of $\bigcup_e P_e$ where $m_{e_0}, m_{e_1}, \ldots$ enumerates all total computable functions $m_i:\mathbb{Q}^{>0}\rightarrow \mathbb{N}$ (this listing will not be computable) and $P_e$ is defined as follows:
\begin{equation*}
P_e = \{ \omega:  \forall \; \epsilon\in \mathbb{Q}\cap (0,1) \; \forall \; n\geq m_e(\epsilon) \; \left| \nu(U\mid [\omega\upharpoonright n])-I_U(\omega)\right|\leq \epsilon\}
\end{equation*}
We argue as follows:
\begin{enumerate}[leftmargin=*]
\item \label{eqn:finally:1} If $m_i(n)\geq m_e(n)$ for all $n\geq 0$, then by definition we have the containment $P_e\subseteq P_i$.
\item \label{eqn:finally:2} For all $0<\delta<1$ there is $i\geq 0$ such that $\nu(P_i)>\delta$. For, since the $\nu$-measure one set $\mathsf{SR}^{\nu}(X)$ is a subset of $\bigcup_e P_e$, there is $k$ such that $\nu(\bigcup_{e\leq k} P_e)>\delta$. Then simply let $m_i=\max_{e\leq k} m_e$, so that $\bigcup_{e\leq k} P_e\leq P_i$. 
\item The set $P_e$ is effectively closed, and indeed is the union of the following two effectively closed sets $C_e$ and $D_e$:
\begin{align*}
C_e & = \{ \omega: \forall \; \epsilon\in \mathbb{Q}\cap (0,1) \; \forall \; n\geq m_e(\epsilon) \; \nu(U\mid [\omega\upharpoonright n]) \geq 1-\epsilon \} \\
D_e & =  \{ \omega: \forall \; \epsilon\in \mathbb{Q}\cap (0,1) \; \forall \; n\geq m_e(\epsilon) \; \nu(U\mid [\omega\upharpoonright n] )\leq \epsilon\}
\end{align*}
\item \label{eqn:finally} There is at least one $e$ such that $\nu(U\cap P_e)<\nu(\mathrm{cl}_X(U)\cap P_e)$. For, by $\nu(U)<1$ and (\ref{eqn:finally:2}), choose $e$ with $\nu(U)<\nu(P_e)$. Then one has $\nu(U\cap P_e)\leq \nu(U)<\nu(P_e)=\nu(\mathrm{cl}_X(U)\cap P_e)$, where the last identity follows since $\mathrm{cl}_X(U)$ by hypothesis has $\nu$-measure one.
\item Since $P_e$ is classically closed and hence a Polish space itself, recall from elementary topology that $\mathrm{cl}_X(U)\cap P_e = \mathrm{cl}_{P_e}(U\cap P_e)$.\footnote{\cite[Theorem 17.4]{Munkres2000-qh}.}
\item One has that $U\cap P_e\subseteq C_e$. For, suppose not: then we would have a $\omega$ in $U\cap P_e$ that was also in $D_e$. Since $U$ is open, choose $n_0\geq 0$ such that $[\omega\upharpoonright n_0]\subseteq U$, so that $\nu(U\mid [\omega\upharpoonright n] )=1$ for any $n\geq n_0$. But then for $n\geq \max(n_0,  m_e(\frac{1}{2}))$ it follows that $\nu(U\mid [\omega\upharpoonright n] )\leq \frac{1}{2}$ since $\omega$ is in $D_e$, which is a contradiction. Hence indeed $U\cap P_e\subseteq C_e$.
\item From the two previous points, $\mathrm{cl}_X(U)\cap P_e = \mathrm{cl}_{P_e}(U\cap P_e)\subseteq \mathrm{cl}_{P_e}(C_e)=C_e$. Hence by taking $\nu$-measure, we have $\nu(\mathrm{cl}_X(U)\cap P_e)\leq \nu(C_e)$. By (\ref{eqn:finally}), we then have at least one $e$ with $\nu(U\cap P_e)<\nu(\mathrm{cl}_X(U)\cap P_e)\leq \nu(C_e)$.
\item But this contradicts that $U\cap P_e$ is equal to $C_e$ on $\mathsf{SR}^{\nu}$:
\begin{itemize}[leftmargin=*]
\item Suppose that $\omega$ is in $\mathsf{SR}^{\nu}$.
\item If $\omega$ is in $U\cap P_e$, then $I_U(\omega)=1$ and so since it is in $P_e$ it is in $C_e$ (by definition of these sets).
\item If $\omega$ is in $C_e$, then $\nu(U\mid [\omega\upharpoonright n])\rightarrow 1$ and since $\omega$ is in $\mathsf{SR}^{\nu}$, we also have by the main Theorem (Theorem~\ref{thm:newnewlevy}) that $\nu(U\mid [\omega\upharpoonright n])\rightarrow I_U(\omega)$, and so $\omega$ is in $U$.
\end{itemize}
\end{enumerate}
\end{proof}



****


\newpage 

% SW working \today

% \begin{thm}\label{thm:rates2}
% Let $X$ be a computable Polish space, and let $\nu$ be a computable point of $\mathcal{P}(X)$. Let $\mathscr{F}_n$ be a full effective filtration, equipped with Kurtz disintegrations.

% Suppose that there is c.e. open $U$ such that $0<\nu(U)<1$ and $\nu(\mathrm{cl}_X(U))=1$.

% Let $f=I_U$ and further suppose that $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n]$ is uniformly usc and hence uniformly computable continuous.

% Suppose $\mathsf{XR}^{\nu}$ is a measure $\nu$-one subset of $\mathsf{KR}^{\nu}$ such that $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)\rightarrow f$ for all $x$ in $\mathsf{XR}^{\nu}$.

% Then it is not the case that for every $x$ in $\mathsf{XR}^{\nu}$ there is a computable function $m:\mathbb{Q}^{>0}\rightarrow \mathbb{N}$ such that for all rational $\epsilon>0$ and all $n\geq m(\epsilon)$ one has $\left|\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)-f(x)\right|<\epsilon$.
% \end{thm}
% \begin{proof}
% Suppose for reductio that $\mathsf{XR}^{\nu}(X)$ is a subset of $\bigcup_e P_e$ where $m_{e_0}, m_{e_1}, \ldots$ enumerates all total computable functions $m_i:\mathbb{Q}^{>0}\rightarrow \mathbb{N}$ (this listing will not be computable) and $P_e$ is defined as follows:
% \begin{equation*}
% P_e = \{ x:  \forall \; \epsilon\in \mathbb{Q}\cap (0,1) \; \forall \; n\geq m_e(\epsilon) \; \left| \mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)-f(x)\right|\leq \epsilon\}
% \end{equation*}
% We argue as follows:
% \begin{enumerate}[leftmargin=*]
% \item \label{eqn:finally:1} If $m_i(n)\geq m_e(n)$ for all $n\geq 0$, then by definition $P_e\subseteq P_i$.
% \item \label{eqn:finally:2} For all $0<\delta<1$ there is $i\geq 0$ such that $\nu(P_i)>\delta$. For, since the $\nu$-measure one set $\mathsf{XR}^{\nu}(X)$ is a subset of $\bigcup_e P_e$, there is $k$ such that $\nu(\bigcup_{e\leq k} P_e)>\delta$. Then simply let $m_i=\max_{e\leq k} m_e$, so that $\bigcup_{e\leq k} P_e\leq P_i$. 
% \item The set $P_e$ is equal to $C_e\cup D_e$, where 
% \begin{align*}
% C_e & = \{ x: \forall \; \epsilon\in \mathbb{Q}\cap (0,1) \; \forall \; n\geq m_e(\epsilon) \; \mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x) \geq 1-\epsilon \} \\
% D_e & =  \{ x: \forall \; \epsilon\in \mathbb{Q}\cap (0,1) \; \forall \; n\geq m_e(\epsilon) \; \mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)\leq \epsilon\}
% \end{align*}
% The set $C_e$ is effectively closed by the hypothesis that $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n]$ is uniformly usc. The set $D_e$ is effectively closed since $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n]$ is uniformly lsc by Proposition~\ref{prop:dis:1}.
% \item \label{eqn:finally} There is at least one $e$ such that $\nu(U\cap P_e)<\nu(\mathrm{cl}_X(U)\cap P_e)$. For, by $\nu(U)<1$ and (\ref{eqn:finally:2}), choose $e$ with $\nu(U)<\nu(P_e)$. Then one has $\nu(U\cap P_e)\leq \nu(U)<\nu(P_e)=\nu(\mathrm{cl}_X(U)\cap P_e)$, where the last identity follows since $\mathrm{cl}_X(U)$ by hypothesis has $\nu$-measure one.
% \item One has that $U\cap P_e\subseteq C_e$. For, suppose not: then we would have a point $x$ in $U\cap P_e$ that was also in $D_e$. Since $U$ is open and the filtration is full, there is an element $A$ in some $\mathscr{F}_{n_0}$ such that $x$ is in $A$ and $A\subseteq U$. Then for all $n\geq n_0$ one has $[x]_{\mathscr{F}_n}\subseteq A$ and hence $\mathbb{E}_{\nu}[I_A\mid \mathscr{F}_{n}](x)=1$ and hence $\mathbb{E}_{\nu}[f\mid \mathscr{F}_{n}](x)\geq \mathbb{E}_{\nu}[I_A\mid \mathscr{F}_{n}](x)= 1$. But then for $n\geq \max(n_0,  m_e(\frac{1}{2}))$ it follows that $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)\leq \frac{1}{2}$ since $x$ is in $D_e$, which is a contradiction. Hence indeed $U\cap P_e\subseteq C_e$.
% \item One has that $U\cap P_e$ is equal to $C_e$ on the $\nu$-measure one set $\mathsf{XR}^{\nu}$:
% \begin{itemize}[leftmargin=*]
% \item Suppose that $x$ is in $\mathsf{XR}^{\nu}$.
% \item If $x$ is in $U\cap P_e$, then $f(x)=1$ and so since it is in $P_e$ it is in $C_e$ (by definition of these sets).
% \item If $x$ is in $C_e$, then $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)\rightarrow 1$ and since $x$ is in $\mathsf{XR}^{\nu}$ we have by hypothesis that $\mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)\rightarrow I_U(x)$, and so $x$ is in $U$.
% \end{itemize}
% \end{enumerate}
% \end{proof}


==> zzz-trash.tex <==
Miyabe has a related translation result for Martin-L\"of tests. For a function $f$ in~$\mathbb{L}_p(\nu)$, one says that $f$ is \emph{weakly $L_p(\nu)$ computable} if there is a computable sequence $f_s$ from the countable dense set of $L_p(\nu)$ such that $f_n\rightarrow f$ on $\mathsf{MLR}^{\nu}$ and $\sum_s \|f_{s+1}-f_s\|^p<\infty$.\footnote{Note that such $f$ are also in $L_p(\nu)$ since $f=f_0+\sum_s (f_{s+1}-f_s)$ on $\mathsf{MLR}^{\nu}$.}$^{,\;}$\footnote{Our definition differs slightly from Miyabe's in that he works just with $p=1$ and he allows for partial functions.} Similar to Proposition~\ref{prop:miyabediff}, one has the following, which extends Miyabe's proof from $p=1$ to $p\geq 1$:\footnote{\cite[Proposition 4.8]{Miyabe2013}.}
\begin{prop}\label{prop:miyabediff2}
Suppose that $\nu$ is a computable point of $\mathcal{P}(X)$ and $p\geq 1$ is computable.
\begin{enumerate}[leftmargin=*]
\item \label{prop:miyabediff2:1} Suppose $f$ is  weakly $L_p(\nu)$-computable point with witness $f_n$. Then there are $L_p(\nu)$ Martin-L\"of tests $g,h$ such that $f=g-h$ on on $\mathsf{MLR}^{\nu}$.
\item \label{prop:miyabediff2:2} Suppose that $g,h$ are $L_p(\nu)$ Martin-L\"of tests. Then there is a weakly $L_p(\nu)$-computable $f$ with witness $f_n$ such that $f=g-h$ on on $\mathsf{MLR}^{\nu}$.
\end{enumerate}
\end{prop}
\begin{proof}
For (\ref{prop:miyabediff2:1}), use the same proof as Proposition~\ref{prop:miyabediff}(\ref{prop:miyabediff:1}).

For (\ref{prop:miyabediff2:2}), suppose that $g_s, h_s$ are the approximations as in Proposition~\ref{prop:exptoflsc}. Without loss of generality $g_0=h_0=0$. Since $g_s\rightarrow g$ in $L_p(\nu)$, choose $s_0\geq 0$ such that for all $s\geq s_0$ one has $\|g_s-g\|_p<\frac{1}{2}$, so that $\|g_{s+1}-g_s\|_p<1$. Since for $y<1$ one has $y\leq y^{\frac{1}{p}}$, one then has the following, using the esimate in Proposition~\ref{prop:estimate}:
\begin{equation*}
\sum_{s\geq s_0} \|g_{s+1}-g_s\|_p \leq \sum_{s\geq s_0} \int (g_{s+1}-g_s)^p\; d\nu \leq  \sum_{s\geq s_0} \int (g_{s+1}^p-g_s^p)\; d\nu = \int g^p - g_{s_0}^p \; d\nu \leq \|g\|_p^p <\infty
\end{equation*}
Hence one has $\sum_s \|g_{s+1}-g_s\|_p<\infty$ and similarly $\sum_s \|h_{s+1}-h_s\|_p<\infty$. Then let $f_s=g_s-h_s$ and let $f=\sum_s f_{s+1}-f_s$ on $\mathsf{MLR}^{\nu}$ and zero otherwise. Then one has $\|f\|_p \leq \sum_s \|g_{s+1}-g_s\|_p+\sum_s \|h_{s+1}-h_s\|_p<\infty$.
\end{proof}

Using this, one can present the following version of Theorem~\ref{thm:drlevy} in terms of weakly $L_p(\nu)$-computable points, provided one assumes that the disintegration is a Martin-L\"of disintegration:
\begin{cor}\label{cor:drlevy}

Suppose that $X$ is a computable Polish space and $\nu$ in $\mathcal{P}(X)$ is computable. Suppose that $\mathscr{F}_n$ is an almost-full effective filtration, equipped uniformly with Martin-L\"of disintegrations~$\rho^{(n)}$.

If $p> 1$ is computable, then the following three items are equivalent for $x$ in $X$: 
\begin{enumerate}[leftmargin=*]
  \item \label{dr:cor:1} $x$ is in $\mathsf{DR}_{\rho}^{\nu}(X)$.
  \item \label{dr:cor:2} $x$ is in $\mathsf{KR}^{\nu}(X)$ and $\lim_n \mathbb{E}_{\nu}[f\mid \mathscr{F}_n](x)=f(x)$ for all weakly $L_p(\nu)$ computable~$f$.
\end{enumerate}
\end{cor}
\begin{proof}
Suppose (\ref{dr:cor:1}); we show (\ref{dr:cor:2}). Sincew we suppose (\ref{dr:cor:1}), we have Theorem~\ref{thm:drlevy}(\ref{dr:thm:2}). Let $f$ be weakly $L_p(\nu)$ computable. By the previous proposition, there are two $L_p(\nu)$ Martin-L\"of tests $g,h$ such that $f = g-h$ on $\mathsf{MLR}^{\nu}$. Since we are working with Martin-L\"of disintegrations, by Proposition~\ref{prop:dis:2}(\ref{prop:newlevy:2a:again}), one has that $\mathbb{E}_{\nu}[f \mid \mathscr{F}_n]=\mathbb{E}_{\nu}[g-h \mid \mathscr{F}_n]$ on $\mathsf{MLR}^{\nu}$ for all $n\geq 0$. Then by Theorem~\ref{thm:drlevy}(\ref{dr:thm:2}) and Proposition~\ref{prop:dis:2}(\ref{prop:newlevy:2c:again}), we have on $\mathsf{MLR}^{\nu}$ that $f=g-h=\lim_n \big(\mathbb{E}_{\nu}[g\mid \mathscr{F}_n]-\mathbb{E}_{\nu}[h\mid \mathscr{F}_n]\big)= \lim_n \mathbb{E}_{\nu}[f\mid \mathscr{F}_n]$. 

Suppose (\ref{dr:cor:2}); we show (\ref{dr:cor:1}). But this follows from Theorem~\ref{thm:drlevy} since every $L_p(\nu)$ Martin-L\"of test is weakly-$L_p(\nu)$ computable. 

\end{proof}
